X-World 1.6: Building Controllable Virtual Cities with World Models

Deploying generative world models for end-to-end closed-loop evaluation and policy learning requires precise scenario control, consistent observations, and sustained generation quality during extended interactions. This report presents X-World 1.6, advancing X-World 1.0 toward a more reliable and versatile driving simulator. The upgraded base model offers finer-grained control over traffic semantics, including traffic lights and road markings, together with improved spatial consistency across cameras. Virtual City capabilities broaden scenario construction through a family of models conditioned on diverse 2D and 3D references, including support for generating multi-camera future videos from a single image. An enhanced post-training framework enables efficient causal, few-step generation with stronger temporal coherence, better quality retention over longer rollouts, and improved alignment with human preferences. We also introduce a dedicated evaluation suite to support systematic assessment and guide model iteration. Together, these upgrades expand the scenarios X-World can simulate and improve the efficiency and reliability of its generated observations, supporting broader use in autonomous-driving development.

==> backup/sections/applications.tex <==
\section{Applications}
X-World 1.0 \cite{xworld2026}demonstrated closed-loop simulation and online reinforcement learning with control over vehicles, lane markings, and curbs. Version 1.6 improves generation, introduces absolute static scene control to preserve the static environment of a selected location, adds control over traffic-light position and color and over road-surface markings, and expands lane-marking and curb categories. Building on the model-capability evaluation in Section \ref{sec:eval}, this section focuses on application-level benefits: how Virtual City supports scenario reuse, closed-loop evaluation and training, and target-behavior reproduction in operational driving tasks.

Virtual City combines location-specific scene records with interactive world-model generation. Within the coverage of existing cloud records, users can select a location and capture time to revisit a scene for simulation or training. The capture time identifies the record; dynamic traffic behavior can vary with the task. Absolute static scene control maintains consistency with the selected scene's road structure, buildings, and other static surroundings throughout generation.

\subsection{Scenario Configuration and Reuse}
A location provides the environmental reference, controls define task conditions, and closed-loop generation enables ongoing policy interaction. Together, they allow the same place to support target-behavior reproduction and policy exploration under different actions. This shared environment connects real-world records to evaluation and training tasks while preserving their scene provenance.

In the proposed platform, a location asset stores scene records and associated information; a scenario configuration specifies the driving task, initial state, and selected conditions; and a generation record links the asset, configuration, generation settings, and multi-camera output. These objects associate multiple tasks with one location and retain input--output relationships for refinement and reuse. Data management, configuration editing, and version associations describe the platform design built on established model capabilities and existing cloud records. Importing additional photographs or street-view material remains a possible extension.

The workflow begins with an existing scene record, an ego starting position, and a driving task. Surrounding-vehicle states or trajectories and relevant lane-marking, curb, road-surface marking, and signal conditions are selected for the task. A left-turn task, for example, can retain the location while varying other vehicles' initial positions and motion to create different encounters. Signal conditions use the currently supported position and color settings. Figure~\ref{fig:vc_scene} illustrates how different interactions share the same static scene reference.

\begin{figure}[tbp]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/virtual_city_scene.pdf}
  \caption{\textbf{Repeated interactions at one location.} This conceptual illustration shows runs sharing a static scene reference while policy actions and dynamic behavior may differ.}
  \label{fig:vc_scene}
\end{figure}

In the proposed workflow, multi-camera outputs generated from a candidate configuration are previewed. Review checks whether fixed structures match the location, vehicles occupy the intended road regions, and visible signal colors and road-surface markings follow the conditions. Views are inspected together, with attention to vehicle motion across cameras and the visibility of key road elements. Where needed, the configuration is revised and regenerated, retaining its conditions and changes from the original.

Selected outputs are linked to their location asset, scenario configuration, and generation settings in this design. Additional recordings extend the scene evidence, while new configurations introduce further traffic tasks at the same location. These associations support inspection and traceability and allow later work to begin from an existing configuration. Reusing a scene provides common experimental conditions; different policy actions can still produce different subsequent observations and trajectories.

\subsection{Closed-Loop Evaluation and Training}
\label{sec:closed-loop-use}
Simulation and reinforcement learning use the same action--observation interface shown conceptually in Figure~\ref{vc_pipeline}. Initial observations, scene conditions, and the ego state define the interaction starting point. The policy receives synchronized multi-camera observations and produces an action or planned trajectory. The simulator advances the ego state accordingly, and the world model generates subsequent observations using the observation history and scene conditions. These observations return to the policy, completing the interaction loop.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/virtual_city_pipeline.pdf}
  \caption{\textbf{Shared interaction pipeline for simulation and RL.} Conceptual illustration of scene-conditioned generation and the policy--environment loop. Interaction records support behavioral evaluation; the RL branch adds training feedback and policy updates.}
  \label{vc_pipeline}
\end{figure}

\textbf{Simulation evaluation.} A simulation begins with a recording segment preceding the target event, giving the policy time to perceive, decide, and respond. The interaction then follows the shared pipeline through the specified evaluation window. Cloud records retain the scene reference as the policy's actions change subsequent observations. The resulting interaction is used to examine reproduction of the target failure behavior, supporting diagnosis and regression evaluation.

\textbf{Reinforcement learning.} RoXDrive~\cite{lin2026roxdrive} provides a public research reference for closed-loop policy optimization with a world model. In this methodological setup, the world model remains frozen while the policy is updated using feedback from interaction. Rewards account for safety, progress, comfort, and centering, connecting the collected rollouts to policy updates. These details describe the public research methodology; they are not presented as the configuration of the internal business training system.

The X-World 1.6 training workflow has run end to end, and internal road testers have reported qualitative improvements in the resulting policy behavior. Quantitative road-test results and business-specific training details are not reported here.

\subsection{Environment Fidelity and Task Support}
\label{sec:environment-evaluation}
Here, we assess X-World 1.6 as a simulation environment for operational driving tasks. We examine agreement with trajectory predictions associated with real-video observations and reproduction of target failure behaviors. Table~\ref{tab:vc_results} summarizes these two comparisons. We then discuss their relevance to operational task demand.

\textbf{Paired-review procedure.} Each comparison pairs the closed-loop results of X-World 1.0 and 1.6 for the same selected test case and target failure behavior. The scene, policy version, task definition, initialization window, and review criteria are aligned across versions. Reviewers compare how faithfully the resulting behavior reproduces the target event, using the original case as the reference.

\textbf{Outcome definitions and aggregation.} Each case receives one of three labels relative to X-World 1.0: \emph{Improved} if 1.6 reproduces the target failure behavior more faithfully, \emph{Comparable} if reproduction is similar, and \emph{Worse} if reproduction is less faithful. Changes in controlled elements or visual quality are recorded separately; better images alone do not count as improved behavioral reproduction. Each reported share is the number of cases assigned to that outcome divided by the total number of reviewed test cases. The three outcomes are mutually exclusive and sum to 100\%; they describe comparative reproduction fidelity, rather than absolute reproduction success rates.

\begin{table}[tbp]
  \centering
  \begin{minipage}{\linewidth}
    \small
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.16}

    % Top-aligned panels share one caption; B includes the review interpretation.
    \begin{minipage}[t]{0.40\linewidth}
      \vspace{0pt}
      \textbf{A. Trajectory consistency}\par\nobreak\vspace{3pt}
      \begin{tabular*}{\linewidth}{@{}l@{\extracolsep{\fill}}r@{}}
        \toprule
        Metric & Change \\
        \midrule
        Mean FDE (relative) & $-20.9\%$ \\
        Share with FDE $<1$\,m & $+5.6$\,pp \\
        Share with FDE $<2$\,m & $+9.4$\,pp \\
        Share with FDE $<5$\,m & $+10.6$\,pp \\
        \bottomrule
      \end{tabular*}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.57\linewidth}
      \vspace{0pt}
      \textbf{B. Paired behavior review}\par\nobreak\vspace{3pt}
      \begin{tabular}{@{}>{\raggedright\arraybackslash}p{20mm}>{\raggedleft\arraybackslash}p{13mm}>{\raggedright\arraybackslash}p{\dimexpr\linewidth-33mm-4\tabcolsep\relax}@{}}
        \toprule
        Outcome & Share & Target behavior \\
        \midrule
        Improved & \textbf{19\%} & More faithful reproduction \\
        Comparable & \textbf{77.4\%} & Similar reproduction \\
        Worse & \textbf{3.6\%} & Less faithful reproduction \\
        \midrule
        \multicolumn{3}{@{}l@{}}{\textbf{Improved or comparable: 96.4\%}\quad\textit{(derived)}} \\
        \bottomrule
      \end{tabular}
    \end{minipage}

    \par\vspace{8pt}
    \footnotesize
    \setlength{\parindent}{0pt}
    \setlength{\parskip}{2pt}
    \textit{A.} pp denotes percentage points; FDE-threshold shares are cumulative.\par
    \textit{B.} Shares use all reviewed cases. The summary combines improved and comparable cases; it is not an absolute reproduction success rate. Visual changes alone do not count as behavioral improvement.
  \end{minipage}
  \caption{Trajectory consistency and target-behavior reproduction: X-World 1.6 versus 1.0.}
  \label{tab:vc_results}
\end{table}

\textbf{Trajectory-level reproduction consistency.} Final displacement error (FDE) measures endpoint discrepancies relative to trajectory predictions obtained from the corresponding ground-truth (GT) videos. In this evaluation, X-World 1.6 reduces mean FDE by 20.9\% relative to 1.0. The percentages of evaluated cases with FDE below 1\,m, 2\,m, and 5\,m increase by 5.6, 9.4, and 10.6 percentage points, respectively. Each percentage is the number of cases satisfying its threshold divided by the total number of evaluated cases; the thresholds are cumulative. These results indicate closer agreement with reference-video trajectory predictions and quantify an aspect of the environment's reproduction fidelity.

\textbf{Behavior-level reproduction.} Reproduction improves in 19\% of test cases, is comparable in 77.4\%, and is worse in 3.6\%. The comparable category can include changes in road structure, signals, markings, or visual quality that do not materially change reproduction of the target failure behavior. It therefore denotes comparable behavioral reproduction, not identical scene appearance. The worse category identifies cases in which 1.6 is less able than 1.0 to reproduce the target behavior.

\textbf{Support for operational task demand.} Virtual City preserves the selected location's road layout, intersection structure, buildings, and static background, providing a stable reference for revisiting target events. Road-surface marking control supplies task-related directional cues, while traffic-signal control supplies conditions for stopping, proceeding, and waiting to turn. Absolute static scene control establishes the spatial setting, and element-level controls specify the traffic conditions within it. Together, they support reproduction in an environment tied to the recorded scene.

To summarize the observed improvements in relation to operational demand, we define a task-demand-weighted reproduction score. Tasks are grouped by their associated controlled elements and mapped to signal-related and road-marking-related groups in the paired review. Their shares of improved reproduction are weighted by internal task demand. By convention, X-World 1.0 is assigned a reference score of 100; each demand-weighted percentage point of improvement adds one score point. The existing mapping gives 1.6 a score of approximately 125, which is retained rather than recomputed from the updated aggregate outcomes in part B of Table~\ref{tab:vc_results}. The score counts improvements without subtracting regressions. It is therefore a descriptive assessment of improvement-related task support, not a net gain after regressions or a measured change in overall reproduction success rate.

The demand mapping has not been validated task by task. The control-dimension groups may overlap, and the evaluation does not isolate the contribution of absolute static scene control or apportion the additional score among individual capabilities. Raw task volumes, weights, and group details remain confidential; these results are not extrapolated to the complete simulation collection.




==> backup/sections/base_model.tex <==
\section{Method}
\label{sec:method}
X-World 1.6 introduces Virtual City Generation as its central capability, extending controllable driving video generation to environments grounded in real-world scenes. The framework combines scene conditioning with scenario control, enabling the same location to support synchronized multi-camera generation under different driving conditions. We first formulate this framework, then describe how visual observations and 3D representations provide scene grounding, and finally present the controls that govern world evolution.

\subsection{From Real-World Scenes to Virtual Cities}
\label{sec:city_formulation}

Driving simulation requires both a persistent environment and a specified evolution of traffic within it. A recorded video couples these two factors to one camera trajectory and one sequence of events. Reusing the underlying location therefore requires recovering scene evidence across viewpoints while controlling which aspects of the recorded scenario are retained or changed. Virtual City Generation addresses this problem through two complementary capabilities: expanding a dashcam recording into synchronized surround views of the same scenario, and generating new scenarios within an environment grounded by reference observations or a 3D representation. We organize these capabilities around
\[
\begin{aligned}
\text{Virtual City}
&= \text{Real-World Scene Grounding} \\
&\quad + \text{Controllable World Evolution}.
\end{aligned}
\]
For independently controlled generation, a scene-grounded Virtual City corresponds to the family of conditional video distributions
\begin{equation}
\mathfrak V_{\mathcal S}
= \bigl\{p_\theta(\,\cdot\mid\mathcal S,\mathcal C,\Pi)
\;:\; (\mathcal C,\Pi)\in\Omega_{\mathcal S}\bigr\},
\label{eq:city_family}
\end{equation}
where $\theta$ denotes the world-model parameters and $\Omega_{\mathcal S}$ comprises scenario and camera configurations compatible with the scene and supported control interfaces. This formulation separates persistent scene evidence $\mathcal S$ from scenario variables $(\mathcal C,\Pi)$, making a location reusable across rollouts. The spatial extent is determined by scene coverage and generative completion; the formulation does not require a complete city-scale reconstruction.

\textbf{Real-world scene grounding defines where.} The scene specification $\mathcal S$ grounds the static-environment component of a Virtual City: road geometry, building arrangement, roadside infrastructure and distinctive surface details. It supplies persistent spatial and visual evidence across cameras and time. Target observations are indexed by
\[
\Pi=\{\pi_t^v\}_{t=1,\ldots,T;\,v=1,\ldots,V},
\qquad
\mathcal Y=\{I_t^v\}_{t=1,\ldots,T;\,v=1,\ldots,V},
\quad V=7,
\]
where $\pi_t^v$ specifies the calibration and pose of camera $v$ at time $t$, and $I_t^v$ is its generated image. As $\Pi$ changes, observed structures should retain compatible projections and newly exposed regions should agree with $\mathcal S$. Regions outside the available coverage are completed using the learned scene prior. Grounding therefore constrains the static environment without prescribing all pixels of its scenario-dependent appearance.

\textbf{Controllable world evolution defines what happens.} We collect the X-World controls as $\mathcal C=(\mathcal A,\mathcal O,\mathcal L,\mathcal F,\mathcal M,\mathcal E)$, representing ego motion, objects, lanes, traffic-light states, road markers and environmental text, respectively. In R2V and controllable 3D-conditioned generation, these signals select a rollout from $\mathfrak V_{\mathcal S}$:
\begin{equation}
\mathcal Y^{(k)}\sim p_\theta\!\left(\,\cdot\mid\mathcal S,\mathcal C^{(k)},\Pi^{(k)}\right),
\qquad k=1,\ldots,K.
\label{eq:virtualcity}
\end{equation}
The scenario index $k$ distinguishes alternative futures with fixed scene evidence $\mathcal S$. Camera configurations $\Pi^{(k)}$ remain consistent with the requested ego motion $\mathcal A^{(k)}$. Scene identity is anchored by structures and details unaffected by the intervention: object edits alter traffic, environmental text changes weather or illumination, and road-semantic edits modify specified static elements. In dashcam generation, the source video fixes both static content and scenario evolution; controllable elements follow that video rather than independently selected interventions.

\textbf{A unified framework for 2D and 3D scene specifications.} We distinguish four input routes within two representation families:
\begin{equation}
\mathcal S\in
\underbrace{\mathbb S_{\mathrm{dashcam}}\cup\mathbb S_{\mathrm{R2V}}}_{\text{2D observations}}
\;\cup\;
\underbrace{\mathbb S_{\mathrm{3DGS}}\cup\mathbb S_{\mathrm{PC}}}_{\text{3D representations}}.
\label{eq:scene_families}
\end{equation}
Here $\mathbb S_m$ denotes the scene-specification space for modality $m$; the four routes are alternative inputs. The framework in Figure~\ref{fig:virtual_city_architecture} comprises scene encoding, geometric association and conditional video synthesis. For 2D inputs, visual features are augmented with GeoPE to express their acquisition geometry in a common scene frame. For 3D inputs, spatial structure provides target-view support: 3D Gaussian scenes supply geometry and reconstructed appearance, while geometry-only point clouds leave appearance to synthesis. Modality-specific conditioning paths supply this evidence to the X-World video backbone alongside the applicable scenario conditions. The generator jointly synthesizes the seven views, combining scene evidence with cross-view and temporal interaction. Dashcam conditions constrain the recorded evolution; R2V and 3D conditions permit scenario selection through $\mathcal C$.

The central design objective is to preserve scene identity under viewpoint change while respecting the appropriate scenario constraints. These requirements define three complementary axes of evaluation: fidelity to observed static content, consistency across views and time, and adherence to source dynamics or requested controls. Visual realism alone does not establish that the generated video represents the specified city or scenario.

\begin{figure}[!thb]
\centering
% Insert the unified Virtual City architecture figure here.
% Example: \includegraphics[width=\linewidth]{figures/virtual_city_architecture.png}
\includegraphics[width=\linewidth]{assets/network_arch.pdf}
\caption{Architecture overview. (a) GeoPE augments scene and video tokens before processing by stacked DiT blocks. (b) Each block integrates scene--video attention, cross-view attention, and conditional inputs. (c) Shared attention allows each view to attend to itself and the scene, while scene queries attend to all views.}
\label{fig:virtual_city_architecture}
\end{figure}

\subsection{Virtual Cities from Visual Observations}

Visual observations instantiate the scene specification $\mathcal S$ in Section~\ref{sec:city_formulation} without requiring an explicit reconstruction. Their central limitation is incomplete spatial coverage: a recorded image supplies detailed appearance within its field of view, but does not directly specify how that content projects into other cameras or what lies behind occlusions. We address this through geometrically indexed visual tokens and their interaction with target-video tokens inside the world model. The two routes impose different constraints on the factorization between scene grounding and world evolution. Dashcam video specifies both the environment and its recorded evolution, making generation a temporally aligned surround-view completion task. R2V supplies reference observations of the environment while retaining $\mathcal C$ as an independent specification of the target scenario. GeoPE provides the common patch-level geometric representation; the conditioning topology determines how each route uses that evidence.

\textbf{Geometry-aware positional encoding (GeoPE).}
GeoPE provides transformer attention with geometric cues for relating
scene observations to target views across cameras and time.
Following the use of camera and ray geometry in positional
encoding~\cite{li2025cameras,wu2026rayrope}, it associates each 2D patch
with a spatially located viewing line and its local angular extent
in a common 3D scene frame.
Camera calibration, distortion correction and pose determine the
patch-center unit direction $\mathbf d$ and camera origin $\mathbf c$,
giving the viewing ray and descriptor
\begin{equation}
\begin{aligned}
\mathbf r(\lambda)
&=\mathbf c+\lambda\mathbf d,\qquad \lambda>0,\\
\mathbf g
&=\bigl[
\mathbf d;\,
\operatorname{symlog}(\mathbf c\times\mathbf d);\,
\Delta\mathbf d_u;\,
\Delta\mathbf d_v
\bigr]\in\mathbb R^{12}.
\end{aligned}
\label{eq:geope_geometry}
\end{equation}
In the Pl\"ucker representation, $\mathbf d$ specifies viewing orientation
and $\mathbf c\times\mathbf d$ encodes the supporting line's spatial
offset; elementwise
$\operatorname{symlog}(x)=\operatorname{sign}(x)\log(1+|x|)$
compresses the moment's dynamic range.
The half-differences
$\Delta\mathbf d_a=\tfrac{1}{2}
(\mathbf d_a^{+}-\mathbf d_a^{-})$, $a\in\{u,v\}$,
describe the patch's horizontal and vertical angular extent, where
$\mathbf d_a^{\pm}$ are unit directions at opposing boundary midpoints
in the same frame.
Together, these terms connect image patches to their 3D viewing
geometry without requiring surface depth.
To retain camera motion within temporally compressed tokens, GeoPE
stores frame-specific descriptors in four ordered slots.
Independently encoded images and the first video latent use only the
first slot; subsequent latents use four consecutive descriptors aligned
with their temporal sampling interval.
A shared two-layer SiLU MLP
$f_\theta:\mathbb R^{12}\rightarrow\mathbb R^{D/4}$
embeds the descriptor $\mathbf g_{ik}$ in slot $k$ of token $i$;
the resulting geometry embedding is fused with visual token
$\mathbf h_i\in\mathbb R^D$ as
\begin{equation}
\begin{aligned}
\mathbf e_i
&=\operatorname{LN}\!\left(
\mathop{\Vert}_{k=1}^{4}
\bigl[m_{ik}f_\theta(\mathbf g_{ik})\bigr]
+E_{\mathrm{support}}(s_i)
+E_{\mathrm{pose}}(v_i)
\right),\\
\widetilde{\mathbf h}_i
&=\mathbf h_i+\mathbf e_i .
\end{aligned}
\label{eq:geope_fusion}
\end{equation}
Here $\Vert$ denotes channel concatenation, $\operatorname{LN}$ denotes
LayerNorm, and $m_{ik}$ masks inactive or pose-invalid slots after the MLP.
The support label $s_i$ indicates one- or four-frame geometry, and the
binary pose-validity label $v_i$ indicates whether camera pose is
available and valid for token $i$.
The learned lookup tables $E_{\mathrm{support}}$ and $E_{\mathrm{pose}}$
map these labels to $D$-dimensional vectors, retaining support and
validity information even when geometric slots are masked.
The same encoder adds $\mathbf e_i$ to both scene-conditioning and noisy
target-video tokens, allowing attention to use appearance together with
viewing geometry when associating scene evidence with target patches.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{assets/geope.pdf}
        \caption{
    \textbf{Geometry-aware positional encoding (GeoPE).}
    \textbf{(a)} Patch descriptors encode ray direction, spatial position,
    and angular extent in a shared 3D frame.
    \textbf{(b)} Shared frame-wise encoding preserves geometric support
    under 1:1 and 4:1 temporal compression through masked, ordered slots.
    \textbf{(c)} State embeddings and LayerNorm produce the GeoPE
    embedding, which is added to the visual token.
    }
    \label{fig:geope}
\end{figure*}

\subsubsection{Dashcam-to-Multi-Camera World Generation}
\label{sec:dashcam}

A dashcam recording observes a driving scenario through a single camera, coupling visible static detail to the ego trajectory, actor motion and environmental conditions of that recording. Extending it to seven views requires both appearance extrapolation and a consistent account of the same events outside the source field of view. In the formulation of Section~\ref{sec:city_formulation}, the dashcam therefore constrains both \emph{where} and \emph{what happens}. Given $\mathcal D=\{D_t\}_{t=1}^{T}$ and target camera configurations $\Pi_{\mathcal D}$ along the recorded trajectory, we generate
\begin{equation}
\mathcal Y_{\mathrm{dash}}\sim p_\theta(\,\cdot\mid\mathcal D,\Pi_{\mathcal D}).
\label{eq:dashcam}
\end{equation}
Static structures, traffic participants, signal states and environmental appearance follow the source video. The generated views extend its spatial coverage while preserving its temporal evolution.

\textbf{Video conditioning as an additional view.} We encode the complete dashcam sequence with the video VAE and patchify its latent representation using the same input projection as the target streams. Let $E_{\mathrm{VAE}}$ denote VAE encoding and $P$ the patch projection. At denoising step $\tau$, the conditioning and target tokens are
\begin{equation}
H_D^0=P\!\left(E_{\mathrm{VAE}}(\mathcal D)\right)+G_D,
\qquad
H_v^0=P(z_\tau^v)+G_v,\quad v=1,\ldots,7,
\label{eq:dashcam_tokens}
\end{equation}
where $G_D$ and $G_v$ are their GeoPE embeddings and $z_\tau^v$ is a noisy target-video latent. The observed dashcam latent enters without diffusion corruption and forms an additional view stream alongside the seven targets. Its latent spatial resolution matches the front-view branch, and its temporal grid remains aligned with the target clip. This retains spatially distributed appearance and motion evidence throughout the observed sequence, instead of reducing the source video to a single global condition.
% Source audit: additional-view topology checked at 2d404d1510d5516b1e81edde7b64b33744dd8e52.
% That commit uses PRoPE. Additive GeoPE here follows the author's explicit
% unified report specification; it is not a claim about that historical commit.

\textbf{Temporal processing and cross-view exchange.} Within each DiT block, spatiotemporal self-attention first processes each view stream. The model then gathers spatial tokens from all views at corresponding latent times for cross-view attention. Denoting the tokens at latent time $t$ in block $\ell$ by $H_{v,t}^{\ell}$, the participating sequence is
\begin{equation}
X_t^{\ell}=\bigl[H_{1,t}^{\ell};\ldots;H_{7,t}^{\ell};H_{D,t}^{\ell}\bigr].
\label{eq:dashcam_exchange}
\end{equation}
Attention over $X_t^{\ell}$ allows every target camera to access the observed view, while per-view temporal processing propagates this information through motion and changing visibility. Camera conditioning and GeoPE distinguish the acquisition geometry of the dashcam from that of the target rig. After cross-view exchange, residual updates and feed-forward layers refine each stream separately. The additional dashcam stream participates throughout the backbone but is removed before the prediction head, so the model outputs only the seven target views. Its hidden features evolve within a denoising pass; the observed latent remains the input condition at subsequent denoising steps.

\textbf{Training pairs and scenario preservation.} Training pairs are constructed from synchronized multi-camera recordings. The front-camera sequence provides a source for dashcam-style augmentation, while the original seven-view recording remains the prediction target. Augmentations vary framing, scale, aspect ratio, image quality and residual distortion, with camera metadata updated to describe the transformed observation. This exposes the conditioning path to source-camera variation while retaining correspondence to a common driving event. The full dashcam sequence supplies the motion context, and the independent ego-action injection is disabled when dashcam conditioning is active. Other supplied conditions must agree with the recorded scenario. Consequently, the learning task is to recover the corresponding surround observations from a restricted view: visible content anchors reconstruction, and the learned prior completes unobserved content under the same scene and event constraints.
% Results and demo: source-aligned seven-view sequences, visibility transitions,
% static-detail retention and actor consistency. Add author-owned evidence here.

\subsubsection{Reference-Enhanced World Generation}
\label{sec:r2v}

Reference observations address a different coverage problem. A target rollout may expose a facade, road-surface pattern or roadside structure that is absent from its initial view but visible in another observation of the same location. R2V makes this additional evidence accessible throughout generation. Let $\mathcal R=\{(R_j,\rho_j)\}_{j=1}^{N}$ contain reference images and their acquisition geometry. The corresponding scene condition $\mathcal S_{\mathcal R}$ instantiates the static-environment component of Section~\ref{sec:city_formulation}, while controls and target cameras select its realization:
\begin{equation}
\mathcal Y_{\mathrm{R2V}}\sim p_\theta(\,\cdot\mid\mathcal S_{\mathcal R},\mathcal C,\Pi).
\label{eq:r2v}
\end{equation}
The references provide place-specific evidence without prescribing a target video timeline. Their capture trajectory and ordering therefore do not determine the generated ego motion or the times at which their content becomes visible.

\textbf{Geometrically indexed reference tokens.} Each reference image is encoded independently by the VAE, preserving its single-frame support, then patchified into the backbone's feature dimension. Its GeoPE embedding uses the reference camera's calibration and pose; target tokens use the requested camera geometry. The input representations take the form
\begin{equation}
H_R^0=\operatorname{Concat}_{j=1}^{N}
\left[P\!\left(E_{\mathrm{VAE}}(R_j)\right)+G_j\right],
\qquad
H_v^0=P(z_\tau^v)+G_v.
\label{eq:r2v_tokens}
\end{equation}
Here concatenation is along the token dimension, and $\mathcal S_{\mathcal R}$ denotes the resulting reference-based condition rather than a reconstructed 3D asset. Appearance features retain local visual detail, while GeoPE locates their observation rays in the same scene frame as the target rays. This gives attention a geometric basis for associating image content across viewpoints without imposing a depth-derived correspondence.

\textbf{A shared reference state with bidirectional attention.} Reference tokens remain an active state through the DiT blocks. Each target camera attends jointly to its own video tokens and the shared reference tokens; the reference state attends to itself and all target cameras. Suppressing block indices, residual paths and output projections, the attention updates are
\begin{equation}
\begin{aligned}
\Delta H_v&=\operatorname{Attn}\!\left(Q_v,[K_v;K_R],[V_v;V_R]\right),\\
\Delta H_R&=\operatorname{Attn}\!\left(Q_R,[K_R;K_1;\ldots;K_7],
[V_R;V_1;\ldots;V_7]\right).
\end{aligned}
\label{eq:r2v_attention}
\end{equation}
Here $Q$, $K$ and $V$ denote learned query, key and value projections. Reference and target projections share the backbone attention weights, and each update normalizes attention jointly over the indicated key sets. Thus, target-video context and reference evidence compete within the same attention operation. A single reference state aggregates information from all cameras and is carried to the next block, rather than evolving as separate camera-specific copies. Together with the backbone's cross-view interaction, this topology exposes the same reference evidence to all target views and allows its representation to adapt as the generated scene develops.

\textbf{Spatial association without a reference timestamp.} Reference-related attention uses spatial positional rotations without a temporal rotation; target-to-target attention retains its spatiotemporal positional encoding. Equation~\ref{eq:r2v_attention} abbreviates these edge-specific positional operations. This preserves temporal organization within each generated video while avoiding an imposed temporal offset between a reference image and the target sequence. Reference modulation uses the clean diffusion timestep, and does not look up a target action at the reference's capture index. Target tokens retain their action-dependent modulation. The reference state may still receive scenario information through joint attention, but its acquisition index does not directly prescribe target motion.

\textbf{Training and controllable generation.} During training, a reference image and its matching camera geometry are sampled from the recorded scene, while the multi-camera video remains the denoising target. Varying the sampled reference position exposes the model to different spatial relations between observed detail and target views. Reference geometry, rather than an assigned output timestamp, determines where that evidence is available to the model. At inference, the references remain fixed while $\mathcal C$ and $\Pi$ specify the requested trajectory, traffic and appearance. The grounding objective is to retain persistent scene detail while allowing reference actors and capture-time lighting to change under those controls. R2V therefore realizes the independently controlled family $\mathfrak V_{\mathcal S_{\mathcal R}}$ introduced in Section~\ref{sec:city_formulation}; dashcam generation instead realizes the recorded scenario through additional cameras.
% Source audit: shared-state attention, edge-specific RoPE and reference action
% decoupling checked against the saved V1.5 source. Its controlled experiment
% uses one same-clip reference. N-reference notation describes the report interface,
% not empirical validation of arbitrary multi-image/cross-clip transfer.
% Results and demo: fixed-reference controlled rollouts, place fidelity,
% reference/geometry ablations and evidence under changed target viewpoints.

\subsection{Virtual Cities from 3D Representations}
\subsubsection{3DGS-Conditioned World Generation}


\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figures/ASC_pipe.pdf}
  \caption{Point-cloud and 3D Gaussian representations for controllable multi-view video generation. The top panel shows the two 3D scene representations with a shared camera trajectory. The bottom rows pair point-cloud and 3D Gaussian references with video outputs, illustrating geometric and appearance cues for controlling scene layout and visual content across views.}
  \label{fig:asc_qualitative}
\end{figure}

A key challenge in video generation is maintaining scene-specific geometry and appearance over extended rollouts. In X-World 1.0, although static road elements (e.g., lane markings and road boundaries) are injected into the video generator, these sparse cues do not fully constrain the surrounding environment, as shown in Fig~\ref{fig:asc_qualitative}. 
As generation proceeds, scene-specific details such as background buildings and guardrail designs may drift from the original scene or become visually inconsistent. This limitation motivates a richer representation that captures not only selected road elements but also the broader geometry and appearance of the environment.




\textbf{3D Gaussian scene representation.} We address this challenge using 3D Gaussian Splatting (3DGS), which provides an explicit 3D representation of static scene geometry and appearance. 
Unlike image-based conditioning, 3DGS enables the same reconstructed scene asset to be rendered along a specified camera trajectory, establishing spatial alignment between the source scene and the target viewpoints before generation. 
The resulting renderings provide geometrically aligned observations of buildings, road surfaces, guardrails, and other reconstructed structures, offering the generator more comprehensive scene-specific evidence throughout the rollout. 

Our objective is to construct an \textit{absolute static scene} that preserves persistent environmental structures while excluding transient objects, e.g., vehicles and pedestrians. 
This separation enables the generator to introduce new traffic participants while maintaining scene-consistent interactions, including the occlusion and reappearance of static structures. 
However, achieving reliable static scene reconstruction is challenging in autonomous driving scenarios, where dynamic objects can contaminate the reconstruction and introduce artifacts into the resulting scene. 
To address this challenge, we adopt two complementary reconstruction strategies depending on the reliability of dynamic-object annotations:

\textit{Dynamic-node modeling.}
Our first strategy follows OmniRe~\cite{chen2025omnire}, which explicitly models dynamic objects as separate nodes from the static environment. By decoupling dynamic instances from persistent scene content, this approach reduces interference from moving vehicles and pedestrians during reconstruction. Since this approach relies on accurate object-level annotations, we use SAM3-based segmentation and tracking to identify dynamic objects and establish their temporal associations. 
We further correct bounding-box offsets introduced by coordinate transformations, track object-associated shadows across frames, and dilate dynamic masks to account for motion blur and uncertain object boundaries. After reconstruction, dynamic nodes can be disabled during rendering, allowing us to obtain the static scene independently of the modeled traffic participants.

\textit{Mask-out static reconstruction.}
When dynamic-object tracking is unreliable, inaccurate instance localization can compromise explicit dynamic modeling. We therefore adopt an alternative strategy that directly excludes dynamic observations from static-scene optimization. Specifically, SAM3-generated masks prevent dynamic regions from contributing to the reconstruction loss:
\begin{equation}
\label{eq:static_reconstruction}
    \mathcal{L}_{\mathrm{static}} = \sum_{t,v} \left\| \mathbf{M}_{t,v}^{\mathrm{valid}} \odot \left( \hat{\mathbf{I}}_{t,v} - \mathbf{I}_{t,v} \right) \right\|_1,
\end{equation}
where $\mathbf{I}_{t,v}$ and $\hat{\mathbf{I}}_{t,v}$ denote the observed and rendered images, respectively, $\mathbf{M}_{t,v}^{\mathrm{valid}}$ identifies pixels eligible for static-scene supervision. By excluding dynamic regions from optimization, this strategy avoids explicitly reconstructing moving objects and focuses the available visual supervision on the persistent environment.

\textit{3DGS Initialization.} 
Since our reconstruction pipeline relies solely on visual observations without ground-truth point clouds, we use random Gaussian initialization by default. As an optional enhancement, we employ Depth Anything 3~\cite{lin2025depth} to estimate a scale-aware sparse point cloud, providing a more informative geometric prior that facilitates convergence and improves reconstruction quality.








\textbf{3DGS-conditioned diffusion training.}
Since each driving sequence provides observations along only a single ego-vehicle trajectory, we use 3DGS to render reference videos along alternative trajectories, enabling the diffusion model to learn from reference static scenes while retaining the original recordings as ground-truth supervision.
Specifically, given a reconstructed scene $\mathcal{S}^{*}$, we render a reference video along trajectory $\boldsymbol{\xi}_{1:T}^{\mathrm{render}}$:
\begin{equation}
    \mathbf{V}^{\mathrm{render}}
    =
    \mathcal{R}\left(
        \mathcal{S}^{*},
        \boldsymbol{\xi}_{1:T}^{\mathrm{render}}
    \right).
    \label{eq:render_condition}
\end{equation}


During training, the X-World action follows the ground-truth trajectory $\boldsymbol{\xi}_{1:T}^{\mathrm{gt}}$, and the original video $\mathbf{V}^{\mathrm{gt}}$ serves as the generation target. The rendered reference provides scene-specific geometric and appearance information, while the action specifies the desired ego motion.
Thus, rendering and generation play complementary roles: 3DGS provides a spatially aligned representation of the static environment, while the generator synthesizes dynamic traffic participants and their temporal evolution in accordance with the specified trajectory. 
Based on real-world ego-driving data, we construct approximately \textit{one million clip} pairs with diverse rendered reference trajectories for diffusion training.


\paragraph{Pose Delta Encoding.}
To account for the discrepancy between the rendered reference trajectory and the X-World action, we analytically compute the per-frame relative pose:
\begin{equation}
    \boldsymbol{\Delta}_t
    =
    \mathbf{M}_0
    \left(\mathbf{C}_t^{\mathrm{gt}}\right)^{-1}
    \mathbf{C}_t^{\mathrm{render}}
    \mathbf{M}_0^{-1},
    \label{eq:pose_delta}
\end{equation}
where $\mathbf{C}_t^{\mathrm{gt}}$ and $\mathbf{C}_t^{\mathrm{render}}$ denote the ground-truth and rendering camera poses, respectively, and $\mathbf{M}_0$ is the inverse of the fixed ego-to-camera extrinsic transformation. The resulting relative transformation is converted into a normalized 6D vector and encoded using Fourier features and a lightweight MLP. The embedding is added to the reference camera's camPE and broadcast to all patches of the corresponding latent frame.

For patch-level geometric conditioning, we incorporate the same pose delta into GeoPE by adjusting the reference view matrix:
\begin{equation}
    \mathbf{W}_{\mathrm{ref}}(t)
    =
    \mathbf{M}_0^{-1}
    \boldsymbol{\Delta}_t^{-1}.
    \label{eq:patch_cape_delta}
\end{equation}
Thus, the relative pose is injected at two complementary levels: camPE encodes it as a learned feature, while GeoPE incorporates it into patch-level camera geometry.
This enables the model to distinguish the viewpoint represented by the reference video from the trajectory specified by the action, rather than simply copying the rendered reference. 
More examples refer to the project page.


\begin{figure}[!t]
  \centering
  \includegraphics[width=0.96\linewidth]{figures/asc_qualitative_figure.pdf}
  \caption{Qualitative comparison of generation without and with absolute static scene (ASC) conditioning, against ground truth. Each row shows one driving scene; \textit{w/o ASC} denotes the base model without 3DGS static-scene conditioning, and \textit{with ASC} denotes our 3DGS-conditioned generation.}
  \label{fig:asc_qualitative}
\end{figure}

\subsubsection{Point Cloud Conditioned World Generation}
\label{sec:pointcloud_world_generation}

We use an absolute static point cloud to ground XWorld generation in a specific location. The point cloud represents persistent structures, including roads, buildings, and roadside objects, in a shared world coordinate system. For a requested ego trajectory, we render this fixed scene into the target camera views at every time step. The resulting conditions specify where observed structures should appear, while XWorld generates complete visual observations and dynamic traffic.

\noindent\textbf{Absolute static scene grounding.}\enspace
Let $\mathcal{P}=\{(\mathbf{x}_j,\mathbf{c}_j)\}_{j=1}^{N}$ denote the static scene point cloud, where $\mathbf{x}_j$ is a world-space position and $\mathbf{c}_j$ is its recorded color. We use the same $\mathcal{P}$ throughout a rollout, providing a shared spatial reference for structures observed across cameras and time. Traffic participants are instead specified through dynamic-object controls and synthesized in the generated video, allowing the same location to support different trajectories and traffic scenarios. For camera $v$ at time $t$, we use its intrinsics $\mathbf{K}_v$ and world-to-camera transform $\mathbf{T}_{t,v}^{c\leftarrow w}$ to render an RGB image $\mathbf{R}_{t,v}$ and an aligned depth image $\mathbf{D}_{t,v}$:
\begin{equation}
    \left(\mathbf{R}_{t,v},\mathbf{D}_{t,v}\right)
    =
    \mathcal{R}
    \left(
        \mathcal{P},
        \mathbf{K}_v,
        \mathbf{T}_{t,v}^{c\leftarrow w}
    \right).
    \label{eq:pointcloud_render}
\end{equation}
Rendering every target frame in all seven views aligns the conditions with the requested video while keeping the underlying scene fixed in world coordinates.

\noindent\textbf{Complementary RGB and depth cues.}\enspace
The RGB render provides coarse color and spatial evidence, but a black RGB pixel is ambiguous: it may depict a dark surface or a location without a projected point. We introduce the aligned depth render to resolve this ambiguity. Zero depth is reserved for pixels without valid point-cloud support; positive values identify projected points and encode their distance. Equivalently, the support mask satisfies $\mathbf{M}_{t,v}(\mathbf{u})=1$ when $\mathbf{D}_{t,v}(\mathbf{u})>0$ and $\mathbf{M}_{t,v}(\mathbf{u})=0$ when $\mathbf{D}_{t,v}(\mathbf{u})=0$. A zero-depth pixel thus means that no point-cloud prior is provided at that image location, rather than asserting that the physical scene is empty. Depth supplies this support information together with geometric ordering, complementing the appearance information in RGB.

\noindent\textbf{Pixel-wise latent injection.}\enspace
We encode the rendered RGB and depth sequences into spatially aligned video latents. At each latent-grid position $p$, we concatenate the noisy video latent and the two condition latents along the channel dimension, then apply a shared linear projector:
\begin{equation}
\begin{aligned}
    \mathbf{h}^{\mathrm{in}}_{t,v,p}
    ={}&
    \mathbf{W}_{\mathrm{proj}}\,
    \operatorname{Concat}_{c}
    \Bigl[
        \mathbf{z}_{\tau,t,v,p},
        \mathcal{E}_{\mathrm{VAE}}(\mathbf{R})_{t,v,p},
        \mathcal{E}_{\mathrm{VAE}}
        \bigl(\mathcal{N}(\mathbf{D})\bigr)_{t,v,p}
    \Bigr]
    +\mathbf{b}_{\mathrm{proj}},
\end{aligned}
\label{eq:pointcloud_conditioning}
\end{equation}
where $\operatorname{Concat}_{c}$ denotes channel-wise concatenation, $\mathcal{N}$ preprocesses depth while preserving zero as the no-point indicator, and $\mathbf{h}^{\mathrm{in}}$ has the channel width consumed by the XWorld DiT. Here ``pixel-wise'' refers to corresponding positions on the video latent grid: each location receives the point-cloud evidence projected to that location. This injection design preserves the spatial correspondence established by rendering. Rather than introducing a separate attention module to associate condition features with video positions, channel concatenation presents the aligned RGB and depth evidence directly at each position. A single shared linear projector performs the required channel mapping, keeping the additional fusion parameters small while enabling XWorld to respond to local point-cloud evidence. Motion, camera, and structured-scene controls continue to provide their respective complementary conditions.

\noindent\textbf{Training and controllable rollout.}\enspace
During training, we render the static point cloud at the camera poses of each target clip and supervise generation with its recorded seven-view video. The RGB and depth renders serve as conditions, while the recorded frames remain the prediction target. At inference time, the requested ego motion determines both the action condition and the poses used in Eq.~\eqref{eq:pointcloud_render}. Keeping them aligned makes the point-cloud evidence correspond to the commanded trajectory. Holding $\mathcal{P}$ fixed while changing the trajectory or dynamic-object controls then produces different rollouts grounded in the same scene.


\subsection{One City, Many Futures}

The scene-input methods described above provide geometric and visual evidence
for a particular location. Building on this evidence, \emph{one city, many futures}
uses the same scene specification to generate alternative driving scenarios
through changes to ego maneuvers, surrounding traffic, or road-element
conditions. The objective is to retain the location's identity while following
the requested interventions, allowing different driving behaviors and traffic
interactions to be examined within a common scene context.

We organize scene controls into ego motion, traffic participants, and
static elements, with environmental text providing appearance guidance:
\begin{equation}
\begin{aligned}
\mathcal C&=(\mathcal A,\mathcal O,\mathcal C_{\mathrm{static}},\mathcal E),\\
\mathcal C_{\mathrm{static}}&=(\mathcal L,\mathcal F,\mathcal M).
\end{aligned}
\end{equation}
Here $\mathcal A$ specifies ego motion and $\mathcal O$ traffic participants.
Static elements comprise continuous geometry, such as lane lines and road
boundaries ($\mathcal L$), and discrete semantic elements, including traffic
lights ($\mathcal F$) and road-marker instances ($\mathcal M$). Static refers
to an element's location in the road environment; a traffic light's state
can still vary over time. Environmental text $\mathcal E$ provides
appearance conditioning. For fixed scene evidence $\mathcal S$,
alternative futures are sampled as
\begin{equation}
\mathcal Y^{(k)}\sim p_\theta
(\mathcal Y\mid\mathcal S,\mathcal C^{(k)},\Pi^{(k)}).
\end{equation}
Target camera configurations $\Pi^{(k)}$ and trajectory-dependent scene
queries change consistently with the requested ego motion; fixing the city
does not require fixing the viewpoint. Visual references constrain the
observed scene content, while 3D representations provide evidence queried
at target poses. Content outside their coverage is completed by the
generator, as discussed in the preceding scene-input sections.

\textbf{Ego motion and traffic participants.} The X-World action interface represents future kinematic states using velocity, curvature, roll, and pitch~\cite{xworld2026}. It applies symlog normalization, Fourier features, and an MLP, combines the result with timestamp embeddings, and injects it through AdaLN-Zero. This provides a concrete conditioning path for future motion. A desired ego trajectory must be expressed consistently in that action representation and in any target poses used to query the scene.

Dynamic-agent conditions use semantic and spatial information. In X-World
1.0~\cite{xworld2026}, category features from the text encoder and
Fourier-encoded coordinates are projected into condition embeddings and
supplied through cross-attention. Modifying the actor configuration need not
replace the scene evidence describing the surrounding location. Time-indexed
object states prescribe motion at their sampling granularity; an initial
object list alone leaves subsequent behavior to generation. Actor trajectories
and traffic-light schedules are specified separately and must be compatible
when constructing coordinated scenarios.

\textbf{Static elements.}
X-World 1.0 supports continuous road geometry, including lane lines and road
boundaries. X-World 1.6 extends these controls to discrete semantic elements:
road markers and traffic lights. Lane conditions describe road organization,
marking instances provide localized semantic cues, and signal conditions
specify light states or schedules. Editing lane or marker geometry changes
the road configuration and may require corresponding changes to the scene
evidence.

\textit{Road-marker conditioning.}
We extend the static-element interface with discrete road-surface markings.
Each marker is represented by category features, sampled geometry, and
adjacent-point offsets, which a dedicated encoder maps to condition tokens.

\textit{Traffic-light conditioning.}
Traffic-light conditioning associates each signal's state with its projected
location in each camera view.
Its color applies to a small camera-specific region and may change within
the four source frames represented by one compressed video latent.
The shared structured branch's token-validity masks do not impose
signal-specific spatial support on its queries; appending color tokens
would therefore not, by itself, localize their direct updates. Applying
the temporal averaging used by the agent and road-marker encoders would
also mix potentially different light states. These spatial and temporal
requirements motivate a dedicated branch for traffic lights, even though
they belong to the static-element category.

We instead encode per-source-frame state tokens and project annotated
signal geometry into each camera using calibration. The projected regions
are pooled to the latent grid to form per-light spatial masks. For spatial
token $p$ and signal $n$, the mask is
\begin{equation}
M^{\mathrm{TFL}}_{v,\ell,f}(p,n)
=\mathbf 1[n\text{ is valid}]
\mathbf 1[p\in\Omega_{v,\ell,f,n}],
\label{eq:many_futures_tfl_mask}
\end{equation}
where $v$ indexes cameras, $f$ indexes the four source-frame slots of latent
step $\ell$, and $\Omega_{v,\ell,f,n}$ is the projected signal region.
A dedicated cross-attention branch follows per-view text attention and
precedes cross-view fusion. Its attention heads are divided into four
groups, each querying the state tokens of its source-frame slot. The first
latent repeats the initial frame across the four slots; subsequent latents
cover four successive frames. Tokens without valid signal support receive
zero direct update from this branch. The design therefore preserves
source-frame state conditioning and explicitly localizes its injection.

\textbf{Shared structured conditioning.}
Agents, road markers, and lanes use separate encoders with independently
learned category projections, geometry projections, and fusion layers.
Each encoder maps its inputs to the common DiT width while retaining a representation tailored to its semantic and geometric
structure. Concatenation preserves these individual representations, providing
a basis for the shared attention layer to distinguish condition types and
select relevant tokens.

At latent step $\ell$, we
combine the encoded tokens and their validity masks as
\begin{equation}
\begin{aligned}
\mathbf H_\ell &=[\mathbf H_\ell^{O}\Vert\mathbf H_\ell^{M}\Vert\mathbf H_\ell^{L}],\\
\mathbf V_\ell &=[\mathbf V_\ell^{O}\Vert\mathbf V_\ell^{M}\Vert\mathbf V_\ell^{L}].
\end{aligned}
\label{eq:many_futures_structured}
\end{equation}
Here $\Vert$ denotes token-axis concatenation after the modality-specific
encoders. Within each DiT block, cross-view self-attention first fuses the
synchronized camera features. These features then query $\mathbf H_\ell$
through one masked cross-attention layer. In 1.0, agents entered a per-view
attention path and lanes used a separate post-fusion branch; 1.6 places all
three structured groups in the shared post-fusion branch. Text remains in
its own per-view context branch. Sharing cross-attention reduces projection parameters and redundant query/output
projection computation across structured conditions.

\textbf{Weather and time of day.}
The text-conditioning pathway retained from 1.0 provides appearance-level
control. In a grounded city, it requests changes to illumination,
visibility, and surface appearance. Reference images and 3DGS renders may
contain conflicting capture conditions, so scene fidelity under
environmental editing cannot mean pixelwise copying. Geometry and
distinctive structures provide the location anchor, while shadows,
reflections, and other condition-dependent attributes can change.

The scene-input routes determine how location-specific evidence enters
generation; the enhanced control interface specifies the requested ego
motion, traffic, road-element states, and appearance. Their composition
realizes the Virtual City
formulation of scene grounding and controllable world evolution, producing
alternative driving scenarios from the same location evidence.
Preservation of scene geometry and visual identity, together with adherence
to these interventions, is assessed by evaluation.

==> backup/sections/conclusion.tex <==
\section{Conclusion, Limitations, and Future Work}
\label{sec:conclusion}

\textbf{Conclusion.}
This report presents X-World~1.6, extending the capabilities of
learned, photorealistic simulation for autonomous driving.
The release introduces finer-grained controls over traffic lights,
road markings, and other driving-relevant scene elements.
By incorporating existing 3D assets as references, it also enables
stronger control over static scene content, connecting explicit
scene specification with photorealistic multi-camera generation.
Improvements in Connected Self Forcing and reinforcement
learning-based post-training further enhance temporal consistency,
action following, and visual quality.
Together, these advances broaden the scenarios that X-World can
represent and improve the generated visual feedback for closed-loop
evaluation and policy learning.

\textbf{Limitations.}
Despite supporting multi-view video rollouts exceeding 30 seconds,
X-World does not yet maintain equally reliable scene memory
throughout extended interactions.
Preserving scene content across prolonged occlusions and long-range
movement remains challenging, and previously observed content may
not be faithfully recovered when it becomes visible again.
Long generation horizons should therefore not be interpreted as
guarantees of persistent spatial and temporal consistency.
The model is also sensitive to the temporal coherence of injected
control conditions.
When these conditions are inconsistent across frames, the generated
observations may exhibit corresponding discontinuities or
inconsistent behavior.
This highlights a remaining limitation in reconciling condition
following with coherent scene evolution under imperfect inputs.

\textbf{Future work.}
We will pursue two complementary directions.
First, we will scale model capacity to strengthen foundational
scene understanding and generation capabilities, providing a
stronger basis for consistent simulation.
Second, we will develop more effective reinforcement learning-based
post-training to jointly improve condition following and temporal
consistency, with particular attention to action adherence and
coherent behavior over extended interactions.
Addressing persistent scene memory and robustness to inconsistent
conditioning will remain important priorities as we advance
X-World toward a more reliable photorealistic simulation environment.
\newpage


==> backup/sections/contributors.tex <==
\section{Contributors}
\label{sec:contributors}

The following individuals contributed to the development of X-World 1.6.
Names are listed alphabetically by given name within each group.

\medskip
\noindent\textbf{Advisors}\\
Xianming Liu, Yu Zhang

\medskip
\noindent\textbf{Project Lead}\\
Boyang Wang

\medskip
\noindent\textbf{Pre-training}\\
Jinhao Deng, Kangjie Chen, Ruixin Liu, Xiangyu Li, Xuejie Lv, Yuqi Zhang

\medskip
\noindent\textbf{Post-training}\\
Chaoda Zheng, Dongbin Zhang, Guangfeng Jiang, Hanlong Chen

\medskip
\noindent\textbf{Simulation and Closed-Loop Policy Training}\\
Kai Yang, Linkun Xu, Shijia Chen, Shuang Deng, Sijia Chen,
Xingjie Liu, Xuezhi Yang, Yuxin Peng

\medskip
\noindent\textbf{Infrastructure}\\
Jianlei Zheng, Yixiao Zeng, Yuecheng Ma

\medskip
\noindent\textbf{Data}\\
Rongliang Cheng, Tianyuan Xie, Xinlong Zheng, Yi Guo

\medskip
\noindent\textbf{TPM}\\
Tenglong (Victor) Gu

\medskip
\noindent\textbf{Additional Contributors}\\
Boyi Sun, Hongbin Lin, Minqi Wang, Puyi Wang, Sin Wai Choo, Yuhao Wang

==> backup/sections/data.tex <==
\begin{figure}[hbp]
    \centering
    \includegraphics[width=\linewidth]{backup/assets/data_final.pdf}
\caption{(a) Data curation through quality filtering, behavior tagging, and scenario selection; flow widths are illustrative. (b) Tag distribution across ego behavior, environment, and conditions; bar lengths indicate within-category percentages.}
    \label{fig:data}
\end{figure}
\section{Data}
\label{sec:data}
Compared with X-World 1.0~\cite{xworld2026}, X-World 1.6 uses a larger pool of real-world driving recordings and a larger training dataset (Section~\ref{sec:data_scaling}). We screen the data for capture defects (Section~\ref{sec:data_cleaning}) and use an expanded set of tags to describe and retrieve driving scenarios (Section~\ref{sec:tag_expansion}). We also construct a dedicated supervised fine-tuning (SFT) dataset through kinematics-based and behavior-based selection (Section~\ref{sec:tag_expansion}). Figure~\ref{fig:data} (a) summarizes the data curation process leading to the SFT dataset.

% \subsection{SFT Data Construction}
% \label{sec:sft_data}
% Compared with X-World~\cite{xworld2026}, X-World~1.6 improves its
% training data in four ways.
% First, we greatly increase the amount of real-world driving
% data (Section~\ref{sec:data_scaling}).
% Second, we add more detailed tags to better describe different
% driving scenarios (Section~\ref{sec:tag_expansion}).
% Third, we build a dedicated supervised fine-tuning (SFT) dataset
% that focuses on scenarios with pronounced ego-vehicle maneuvers
% and key driving behaviors (Section~\ref{sec:sft_data}).
% Finally, we clean the data by identifying and removing samples
% with errors introduced during data collection
% (Section~\ref{sec:data_cleaning}).

\subsection{Data Scaling}
\label{sec:data_scaling}
Both X-World 1.0~\cite{xworld2026} and X-World 1.6 build their training datasets by selecting clips from a larger pool of real-world driving recordings. Compared with X-World 1.0, X-World 1.6 uses a candidate pool four times as large and a training dataset twice as large. This allows us to train on more data while being more selective about which clips to include.
%
For a given scenario, the larger pool offers more clips to choose from, allowing us to apply stricter quality criteria while retaining enough training data. It also provides more examples of less common driving behaviors and challenging scenarios, making it easier to broaden scenario coverage without relying heavily on repeated sampling of a small set of clips. We select the training data using the cleaning pipeline in Section~\ref{sec:data_cleaning} and the expanded tagging system in Section~\ref{sec:tag_expansion}. The cleaning pipeline removes recordings with capture errors or other quality issues, while scenario tags help us control the mix of scenarios in the final dataset.


\subsection{Data Cleaning}
\label{sec:data_cleaning}

Multi-camera driving recordings can contain defects introduced during data capture, including luminance flicker, color stripe artifacts, and degraded image quality in individual camera streams. These defects may degrade the quality of generated videos, as the model can learn to reproduce them during training. We therefore exclude affected clips from the training set. We detect each type of issue on a per-window basis. All detection thresholds were calibrated by manually reviewing flagged samples and samples near each threshold.

\textbf{Luminance Flicker.}
\label{sec:flicker}
Flicker appears as abrupt frame-to-frame brightness jumps, typically caused by exposure control or by interference with artificial light sources. Let $Y_c(t)$ be the mean luminance of camera $c$ at frame $t$. We measure flicker by the mean magnitude of the second-order temporal difference, maximized over cameras, as given in Eq.~\eqref{eq:flicker}:
\begin{equation}
\mathrm{osc} = \max_{c} \; \frac{1}{T-2} \sum_{t=2}^{T-1} \Bigl| Y_c(t) - \tfrac{1}{2}\bigl(Y_c(t-1) + Y_c(t+1)\bigr) \Bigr|.
\label{eq:flicker}
\end{equation}
The second-order difference vanishes for gradual illumination changes, such as entering a tunnel, while it responds strongly to isolated brightness spikes. We exclude a video segment from the training set if its $\mathrm{osc}$ value exceeds the threshold $\tau_{\mathrm{osc}}$.

\textbf{Color Stripe}.
\label{sec:striping}
Color stripe artifacts appear as horizontal colored bands caused by sensor or transmission faults. These bands produce stronger color changes between adjacent rows than between adjacent columns, without similarly strong changes in brightness. We use $c = R - G$ as a color-difference signal and $y = (R + G + B)/3$ as a brightness estimate. For each frame, we compute a stripe score $s$:
\begin{equation}
s = \frac{\overline{|\Delta_{\mathrm{row}}\, c|}}{\overline{|\Delta_{\mathrm{col}}\, c|}} \cdot \frac{\overline{|\Delta_{\mathrm{row}}\, c|}}{\overline{|\Delta_{\mathrm{row}}\, y|}},
\label{eq:stripe}
\end{equation}
where $\Delta_{\mathrm{row}}$ and $\Delta_{\mathrm{col}}$ denote differences between adjacent rows and adjacent columns, respectively, and the overbar denotes a spatial mean. The first ratio compares color changes between rows with those between columns. The second compares color changes with brightness changes between rows, helping distinguish color stripe artifacts from ordinary horizontal structures such as road edges. We flag a temporal window if the stripe score exceeds the threshold $\tau_s$ in every frame.

\textbf{Degraded Image Quality}.
\label{sec:degraded_quality}
Degraded image quality refers to reduced scene visibility, a strong global color cast, or overexposure, excluding the luminance flicker and color stripe artifacts discussed above. Reduced visibility can result from a fogged, dirty, or partially obstructed lens. Our screening relies on a key assumption: within a temporal window, these issues typically affect only one or a few cameras, while most camera streams remain unaffected. We therefore compare camera views to identify potentially affected streams. We use two stages: candidate screening designed for high recall, followed by verification with a vision--language model (VLM).

\paragraph{Candidate screening.}
Let $g_c$ denote the texture energy of images from camera $c$. Scene conditions such as fog, rain, and low light can reduce texture across multiple camera views. To account for these shared effects, we flag the stream from camera $c$ for low texture only when its texture energy is low both in absolute terms and relative to the other cameras:
\begin{equation}
g_c < g_{\min} ;\wedge; \frac{g_c}{\operatorname{median}{c' \neq c}, g{c'}} < \tau_1 ;\wedge; \frac{g_c}{g_{\pi(c)}} < \tau_2,
\label{eq}
\end{equation}
where $\pi(c)$ denotes the other camera whose viewing direction is closest to that of camera $c$. The last condition helps avoid false alarms when both views have similarly low texture, which may reflect shared scene content or environmental conditions. We also flag streams whose images have a strong global color cast or are overexposed.


\subsection{Tag Expansion}
\label{sec:tag_expansion}
In this release, we expand the annotation taxonomy to more than 150 tags, with additions focused on data quality, fine-grained agent behaviors, and corner cases. Quality tags indicate potential data quality issues. More detailed behavior tags distinguish interactions and maneuvers that were previously grouped under broader labels, while corner-case tags support targeted retrieval of uncommon and challenging situations. The expanded taxonomy allows us to identify and select a wider range of scenarios from the candidate pool.

We also improve annotation accuracy by refining the tagging algorithms. Incorrect tags can introduce irrelevant samples into a selected category, while missed labels can leave important scenarios underrepresented. Broader tag coverage and more accurate annotations make the larger candidate pool more useful for targeted retrieval and provide finer control over the composition of the selected data. The same annotations support the behavior-based SFT selection described next.

\subsection{SFT Data Construction}
\label{sec:sft_data}
We construct the SFT dataset from candidate driving data retained after the cleaning procedures in Section~\ref{sec:data_cleaning}. The natural distribution of driving data is highly imbalanced: lane keeping and steady cruising dominate, while sharp turns, stops, and lane changes are less frequent. Uniformly sampling windows from this distribution provides limited supervision for these less common maneuvers. We therefore use two complementary selection strategies, based on ego-vehicle kinematics and annotated behaviors, to increase their representation in the SFT data.

\textbf{Kinematics-based selection.}
We examine the ego-vehicle trajectory within each temporal window. Windows with sustained high path curvature capture lateral maneuvers, such as turns at intersections. Windows in which the vehicle decelerates from motion to a complete stop capture longitudinal maneuvers. These criteria select examples directly from the recorded ego motion.

\textbf{Behavior-based selection.}
Kinematic criteria describe vehicle motion but do not by themselves identify the scene context or interactions in which it occurs. We therefore use behavior tags to select events such as turning through an intersection, merging at a lane split, and overtaking a slower vehicle. Because a single clip may contain several occurrences of the same behavior, we treat each tag instance, rather than each clip, as a sampling unit. 
%
We use category-specific resampling ratios to favor scenarios with richer interactions, such as those at intersections. Figure~\ref{fig:data} (b) presents selected tag distributions in the SFT dataset, covering ego behavior, environment, and driving conditions.

% The natural distribution of driving data is highly imbalanced. Lane keeping and steady cruising dominate, while sharp turns, stops and lane changes are comparatively rare. A model fine-tuned on uniformly sampled windows therefore receives little supervision on exactly the scenarios in which action-conditioned generation is most challenging. We construct the SFT set from two complementary sources: windows selected by ego-vehicle kinematics, and windows selected by annotated behaviors.

% \paragraph{Kinematics-based mining.}
% From the ego trajectory of each window, we select windows with sustained high path curvature, which capture lateral maneuvers such as intersection turns, and windows in which the vehicle decelerates from motion to a complete stop, which capture longitudinal maneuvers.

% \paragraph{Behavior-based mining.}
% Kinematic criteria cannot express behaviors defined by the surrounding scene, such as turning through an intersection, merging at a lane split, or overtaking a slower vehicle. For these we rely on the behavior tags. Because a clip may contain several instances of the same behavior, we treat each tag instance, rather than each clip, as a sampling unit, and resample each behavior category with a category-specific ratio that favors interaction-rich scenarios such as intersections.



==> backup/sections/eval.tex <==
\section{Evaluation}
\label{sec:eval}

Evaluating a driving world model requires judging the visual fidelity of the generated multi-camera videos, their adherence to the action condition, and their consistency over time and across views. Human evaluation provides the reference judgment of generation quality (Section~\ref{sec:human_eval}). Because human evaluation is costly, we train a VLM evaluator that localizes anomalies in generated videos and serves as a first pass before human verification (Section~\ref{sec:vlm_eval}). We evaluate action adherence with an inverse dynamics model (IDM) (Section~\ref{sec:idm_eval}), and use an automated consistency benchmark to compare model versions and training variants (Section~\ref{sec:consistency_eval}).

\subsection{Human Evaluation}
\label{sec:human_eval}
We evaluate generation quality using a structured, anomaly-based human assessment protocol. Each generated sequence is reviewed across all seven camera views, with failures localized by image region and temporal interval. These annotations support video-level quality assessment while retaining the evidence needed to distinguish different failure modes.
Our evaluation covers four complementary aspects. Visual fidelity captures image degradation, including blur, excessive sharpening, color distortion, and frame-level discontinuities. Scene consistency assesses the geometric plausibility and temporal persistence of static structures, as well as agreement between camera views observing the same scene. Dynamic plausibility evaluates the shape, identity, and motion continuity of surrounding agents, penalizing artifacts such as spontaneous appearance or disappearance, object merging, and physically implausible interactions. Condition adherence assesses whether generated content agrees with available control annotations, including object locations, lane geometry, road-marking semantics, and traffic-light states. These checks complement the dedicated ego-action evaluation in Section~\ref{sec:idm_eval}.
Annotators record each failure over its affected frames, distinguishing generation errors from legitimate occlusion and viewpoint changes. When multiple artifacts arise from the same underlying event, the primary failure is annotated to avoid redundant penalties. Video-level assessment aggregates anomaly penalties with weights reflecting camera priority, object size, and relevance to the driving region. This weighting emphasizes errors that are visually prominent or directly affect the ego vehicle’s surroundings. A separate quality-control stage audits sampled annotations and requires correction when discrepancies materially change the resulting scores or rankings. The resulting human judgments provide the reference for generation quality, while the localized annotations support anomaly detection and verification in Section~\ref{sec:vlm_eval}.

% TODO: GTA human evaluation

\subsection{VLM-based Evaluation}
\label{sec:vlm_eval}

Human evaluation of generated multi-camera videos is accurate but costly: an annotator must inspect every camera over every frame and localize each artifact with a bounding box. To improve evaluation efficiency, we adopt a coarse-to-fine protocol in which a vision--language model (VLM) first proposes candidate anomalies, and human annotators then verify and refine them instead of annotating from scratch. Following CaC~\cite{wang2026cac}, we formulate the task of the VLM as spatiotemporal anomaly localization, so that its predictions share the format of human annotations and can be checked against them directly.

\subsubsection{Task Formulation}
\label{sec:vlm_task}

Given one camera view of a generated video, the evaluator predicts (i) a binary status indicating whether the view contains any anomaly; (ii) the set of anomaly categories present, drawn from the taxonomy of the human evaluation protocol, which covers image quality, static objects, dynamic objects and controllability; and (iii) for each anomaly instance, its temporal extent as start and end frame indices together with its bounding boxes, in coordinates normalized to $[0, 1000]$ within the camera view. This output matches the granularity of human annotation, so each prediction can be accepted, corrected or rejected by an annotator.

\subsubsection{Training}
\label{sec:vlm_training}

\paragraph{Training data.}
We start from human annotations of generated videos and expand them with a model-in-the-loop procedure: the current evaluator pre-labels new videos, annotators correct its predictions, and the corrected samples are added to the training set. Normal and abnormal samples are kept balanced, and training and evaluation data are split by scene, so that videos generated from the same scene never appear in both.

\paragraph{Supervised fine-tuning.}
Starting from Qwen3-VL-8B-Instruct~\cite{bai2025qwen3vl}, we first fine-tune on single frames, so that the model learns to recognize and box anomalies that are identifiable within one frame. We then fine-tune on video clips, so that it learns to predict anomaly categories, temporal extents and per-frame boxes jointly.

\paragraph{Reinforcement learning.}
We further optimize the evaluator with GRPO~\cite{shao2024deepseekmath}, using a reward that measures how well a prediction matches the annotation, defined in Eq.~\eqref{eq:vlm_reward}:
\begin{equation}
R = w_1 R_{\mathrm{fmt}} + w_2 R_{\mathrm{stat}} + m \left( w_3 R_{\mathrm{type}} + w_4 R_{\mathrm{temp}} + w_5 R_{\mathrm{spa}} \right),
\label{eq:vlm_reward}
\end{equation}
where $R_{\mathrm{fmt}}$ rewards a valid output format, $R_{\mathrm{stat}}$ a correct status, $R_{\mathrm{type}}$ the overlap between predicted and annotated categories, $R_{\mathrm{temp}}$ the IoU between predicted and annotated anomalous frames, and $R_{\mathrm{spa}}$ the mean box IoU on frames where both are present. The indicator $m$ is 1 for abnormal samples and 0 for normal ones. The localization terms receive the largest weights, so that the evaluator is rewarded for pointing to the right place and time, not only for the right verdict.

\subsubsection{Results}
\label{sec:vlm_results}

We measure the efficiency gain on 150 generated videos by comparing two annotation workflows: annotating each video from scratch, and correcting the pre-labels produced by the evaluator. With pre-labeling, the time required to annotate all 150 videos decreased from 2 days to 1 day, a reduction of 50\%.

\subsection{Action Evaluation with IDM}
\label{sec:idm_eval}

% % TODO: IDM-based action evaluation


\subsection{Temporal and Cross-View Consistency Evaluation}
\label{sec:consistency_eval}

Plausible individual frames do not ensure that generated videos describe a coherent evolving scene. Objects may change appearance over time, textures may flicker, and observations from different cameras may imply incompatible spatial configurations. Such failures become particularly relevant when a model generates successive chunks from its own history, where local errors can persist or accumulate. We build an automated benchmark with three complementary modules: object tracking, compression-based temporal evaluation, and reconstruction. Together, they examine object appearance, temporal predictability, and geometric reconstructability to compare X-World~1.0 with the SF and CSF variants of X-World~1.6.% Together, they examine object appearance, temporal predictability, and geometric reconstructability to compare X-World~1.0 with the current model's Self Forcing (SF), Connected Self Forcing (CSF), and long-horizon tuning variants.

For a scene, the benchmark takes synchronized generated frames $\{I_t^v\}_{t=1,v=1}^{T,V}$ and the corresponding camera calibration, where $T$ is the number of frames and $V$ the number of views. The generated videos themselves serve as the inputs to the diagnostic procedures; no paired real-video target or manual object-identity annotation is required. This makes the benchmark applicable to different generated futures under the same scene conditions. Its scores characterize internal consistency and complement visual-quality and action-adherence evaluation.

\subsubsection{Consistency Metrics}
\label{sec:consistency_metrics}

\paragraph{Object tracking consistency.}
We use SAM~3~\cite{carion2025sam3} for text-prompted object detection and segmentation and ByteTrack~\cite{zhang2022bytetrack} to associate detections within each view. Masked object crops are encoded by FG-CLIP~2~\cite{xie2025fgclip2}, producing normalized appearance embeddings $\mathbf e_{k,t}$ for track $k$ at frame $t$. Masking reduces background influence, so the comparison focuses on object appearance rather than the surrounding scene. A continuity gate excludes observations whose appearance and geometric continuity indicate unreliable association, missing observations are not interpolated for appearance scoring.

For frame intervals $\delta\in\mathcal D=\{1,2,4,8,16,32\}$, we compare embeddings from the same track. Let $\mathcal P$ contain all valid triples $(k,t,\delta)$ for which both observations are available. Mean Appearance Consistency is
\begin{equation}
    C_{\mathrm{app}}=
    \frac{1}{|\mathcal P|}\sum_{(k,t,\delta)\in\mathcal P}
    \mathbf e_{k,t}^{\top}\mathbf e_{k,t+\delta}.
    \label{eq:wm_appearance_consistency}
\end{equation}
Higher similarity indicates more stable object appearance across the evaluated intervals. The score normalizes by the number of compared pairs, giving greater weight to tracks with more valid observations. The intervals are measured in frames and correspond to $\delta/f$ seconds at frame rate $f$, which is fixed across checkpoint comparisons.

To distinguish similar average scores with different temporal behavior, we also measure how similarity changes as the frame interval increases. For each track, let $\bar c_k(\delta)$ be its mean similarity at interval $\delta$, and let $\mathcal D_k$ contain the intervals with valid samples. We fit
\begin{equation}
    (a_k,b_k)=\underset{a,b}{\operatorname{arg\,min}}
    \sum_{\delta\in\mathcal D_k}
    \left[\bar c_k(\delta)-a-b\log_2\delta\right]^2,
    \qquad
    D_{\mathrm{app}}=\frac{1}{|\mathcal K|}\sum_{k\in\mathcal K}b_k,
    \label{eq:wm_appearance_decay}
\end{equation}
where $\mathcal K$ contains tracks with at least two distinct valid intervals. Mean Appearance Decay Rate $D_{\mathrm{app}}$ describes the change in similarity when the interval doubles. A negative slope indicates decay, and a slope closer to zero indicates slower decay. This complements the mean score: persistent appearance drift may reduce similarity more strongly at larger intervals even when adjacent frames remain similar.

For cross-view evaluation, same-category tracks are associated using calibrated rays through mask centroids. Let $\mathbf o_a,\mathbf o_b$ denote camera centers in a common ego coordinate system and $\mathbf d_a,\mathbf d_b$ the unit viewing directions of a matched observation pair $p$. Its geometric residual and the scene-level Mean Ray Residual are
\begin{equation}
    r_p=\min_{s,u\in\mathbb R}
    \left\|\mathbf o_a+s\mathbf d_a-\mathbf o_b-u\mathbf d_b\right\|_2,
    \qquad
    R_{\mathrm{ray}}=\frac{1}{|\mathcal Q|}\sum_{p\in\mathcal Q}r_p,
    \label{eq:wm_ray_residual}
\end{equation}
where $\mathcal Q$ contains associated same-frame observations from different cameras with non-parallel rays and closest points in front of both cameras. The residual is measured in meters. Lower values indicate better geometric agreement among the matched views. Because association itself uses geometric compatibility, this is a conditional diagnostic of matched objects; its interpretation should also consider cross-view observation coverage.

\paragraph{Compression-based temporal consistency.}
Earlier work studies flickering in predictively coded video~\cite{pandel2008flickering}. Recent analysis further reports that unpredictable dynamics suffer greater compression-induced temporal instability than larger, structured motion~\cite{zsoldos2026compression}, motivating temporal predictability as a diagnostic signal. A complementary approach, Video Consistency Distance (VCD), measures frequency-domain distances between conditioning-image and generated-frame features and uses them for reward-based I2V fine-tuning~\cite{aoshima2025vcd}.

We measure temporal predictability through the gain from H.264 inter-frame prediction (Fig.~\ref{fig:compression_consistency}). Motion-compensated prediction exploits recurring content across frames, whereas irregular changes require additional residual coding. Each video is encoded twice with the same encoder and quality setting: once with a long GOP and once with all-intra coding. The all-intra stream provides a spatial coding baseline for the same content. We fix the encoder to libx264, CRF~36, and an inter-frame GOP length of~128, disabling adaptive scene-cut insertion to keep the GOP structure controlled.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/compression_consistency_vector.pdf}
    \caption{\textbf{Compression-based temporal consistency.} (a) Inter-frame and all-intra coding of the same video provide quality gains and an encoded-size ratio. (b) Conceptual illustration of larger prediction residuals from irregular appearance changes under the same motion.}
    \label{fig:compression_consistency}
\end{figure}

Let $S_{\mathrm{inter}}$ and $S_{\mathrm{intra}}$ denote the mean frame-wise SSIM of the decoded streams against the input video, and $P_{\mathrm{inter}}$ and $P_{\mathrm{intra}}$ the corresponding PSNR values. Both are computed on the luminance channel. With $B$ denoting encoded file size, the three metrics are
\begin{equation}
    \Delta\mathrm{SSIM}=S_{\mathrm{inter}}-S_{\mathrm{intra}},
    \qquad
    \Delta\mathrm{PSNR}=P_{\mathrm{inter}}-P_{\mathrm{intra}},
    \qquad
    R_{\mathrm{bits}}=\frac{B_{\mathrm{inter}}}{B_{\mathrm{intra}}}.
    \label{eq:wm_compression_consistency}
\end{equation}
Larger quality gains indicate greater benefit from temporal prediction. Since the two streams have identical duration, the encoded-size ratio also represents their average bitrate ratio; lower values indicate more efficient inter-frame coding. We use it as an auxiliary signal alongside the quality gains. Comparing against the intra baseline reduces sensitivity to spatial complexity, but does not fully remove dependence on motion or content. These metrics therefore assess predictability under a fixed codec configuration, with checkpoint comparisons performed on matched scenes and generation conditions.

\paragraph{Reconstruction consistency.}
We use UniSplat~\cite{shi2026unisplat} as a fixed feed-forward 4D reconstruction model to probe both cross-view and temporal consistency. Incompatible observations across cameras or abrupt changes in object appearance over time can disrupt reconstruction through a shared spatial representation with temporal memory, producing flicker, sudden changes, or reconstruction errors in the re-rendered videos. Synchronized multi-view frames are processed jointly at each time step and sequentially over time, retaining the model's internal Gaussian history to incorporate previous observations. The reconstruction is rendered at the supplied camera poses without pose refinement, so camera calibration remains a fixed constraint throughout evaluation. Abstractly, the procedure is
\begin{equation}
    (\mathcal G_t,h_t)=F_{\mathrm{rec}}(\{I_t^v\}_{v=1}^{V},\mathcal C,h_{t-1}),
    \qquad
    \hat I_t^v=\mathcal R(\mathcal G_t;\mathcal C_v),
    \label{eq:wm_reconstruction}
\end{equation}
where $\mathcal C$ denotes camera calibration, $h_t$ temporal memory, $\mathcal G_t$ the current reconstructed Gaussian representation, and $\mathcal R$ the renderer. This allows the representation to evolve with the scene while using historical information. The evaluation compares reconstructions at observed views rather than measuring held-out novel-view synthesis.

Rendered and input frames are compared at the reconstruction resolution. For an aligned pair of decoded RGB frames $x,y$ in the 8-bit pixel domain, we report SSIM together with
\begin{equation}
    \mathrm{PSNR}(x,y)=10\log_{10}
    \frac{255^2}{\frac{1}{N}\sum_{i=1}^{N}(x_i-y_i)^2},
    \qquad
    \mathrm{MAE}(x,y)=\frac{1}{N}\sum_{i=1}^{N}|x_i-y_i|,
    \label{eq:wm_reconstruction_errors}
\end{equation}
where $N$ counts all pixel-channel values. SSIM measures local structural agreement, PSNR summarizes squared pixel error in dB, and MAE reports absolute error in pixel intensity units. Higher SSIM and PSNR and lower MAE indicate better reconstruction fidelity, which serves as a proxy for cross-view and temporal consistency. We first average frame-level scores within each view, then average across views. Using the generated input as the reference tests reconstructability rather than agreement with a real future. The scores depend on both scene consistency and the fixed reconstruction model's capacity and priors, providing complementary evidence to tracking and compression.

\subsubsection{Evaluation Protocol}
\label{sec:consistency_protocol}

For checkpoint comparisons, we fix the scene set, conditioning inputs, camera calibration, resolution, frame rate, rollout duration, and random seeds. Sampling configurations are controlled within each comparison and documented when they differ across stages. Evaluator weights and codec settings remain fixed across checkpoints. Compression and reconstruction scores are averaged over camera views within each scene; tracking scores aggregate valid observations as defined above. For a metric $m$ and checkpoints $A,B$, dataset-level scores and paired changes are
\begin{equation}
    \bar m_A=\frac{1}{|\mathcal S|}\sum_{s\in\mathcal S}m_A(s),
    \qquad
    \Delta\bar m_{A,B}=\frac{1}{|\mathcal S|}\sum_{s\in\mathcal S}
    \left[m_A(s)-m_B(s)\right],
    \label{eq:wm_scene_aggregation}
\end{equation}
where $\mathcal S$ contains scenes with a valid value of $m$ for both checkpoints. Equal scene weights prevent scenes with more frames or detected objects from dominating the dataset-level comparison. Scenes without valid observations for a tracking metric are marked unavailable rather than assigned a perfect score; their counts must be reported alongside the comparison.

The planned analysis will also record valid track and cross-view pair coverage and compare early, middle, and late temporal windows. These checks distinguish changes in evaluation coverage from changes in consistency and assess degradation with rollout position beyond appearance decay across frame intervals. Temporal windows will use the same boundaries for all compared checkpoints, enabling the analysis to identify whether improvements persist into the later parts of a generated sequence.

% \subsubsection{Comparison with X-World~1.0 and Training Variants}
\subsubsection{Comparison between X-World Variants}
\label{sec:consistency_results}

Table~\ref{tab:consistency_stages} compares X-World~1.0~\cite{xworld2026} with four variants of the current model: SF, CSF, SF+LongTuning, and CSF+LongTuning. All nine metrics are reported, together with their equally weighted average rank across the five models. Each metric is ranked according to its preferred direction, with average ranks assigned to ties.

\paragraph{SF, CSF, and long-horizon tuning.}
CSF improves object appearance and cross-view agreement over SF, while reconstruction scores remain mixed. CSF+LongTuning achieves the best average rank, the slowest appearance decay, and the best scores on all three compression metrics. Its stronger temporal predictability is consistent with CSF's cross-chunk feedback (Sec.~\ref{sec:connected_self_forcing}), which optimizes earlier chunks for their contribution to future predictions. Relative to CSF, long-horizon tuning improves compression and reconstruction, with small regressions in mean appearance consistency and ray residual. SF+LongTuning retains better ray agreement and reconstruction fidelity.

Fig.~\ref{fig:sf_csf_compare} complements the quantitative comparison with qualitative examples of SF and CSF, highlighting differences in the preservation of scene details over extended rollouts.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/SF_CSF_Compare.pdf}
    \caption{Qualitative comparison of temporal consistency between Self Forcing (SF) and Connected Self Forcing (CSF). Each pair of rows shows synchronized frames from SF (top) and CSF (bottom). From top to bottom, the examples compare vehicle appearance, sky color, gate details, and road structure. Blue and orange boxes mark selected earlier and later regions, respectively, with corresponding enlarged views and timestamps shown in the rightmost column.}
    \label{fig:sf_csf_compare}
\end{figure}

\paragraph{Comparison with X-World~1.0.}
CSF+LongTuning improves all tracking and compression metrics, as well as reconstruction SSIM, over X-World~1.0. The latter retains better reconstruction PSNR and MAE. The overall gains therefore favor object consistency and temporal predictability, with a remaining trade-off in pixel-level reconstruction fidelity.

\begin{table}[htbp]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{lcccccccccc}
        \toprule
        & \multicolumn{3}{c}{Tracking} & \multicolumn{3}{c}{Compression} & \multicolumn{3}{c}{Reconstruction} & Overall \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-11}
        Model / Variant & App. $\uparrow$ & Decay $\uparrow$ & Ray $\downarrow$ & $\Delta$SSIM $\uparrow$ & $\Delta$PSNR $\uparrow$ & Bits $\downarrow$ & SSIM $\uparrow$ & PSNR $\uparrow$ & MAE $\downarrow$ & Avg. Rank $\downarrow$ \\
        \midrule
        X-World 1.0 & 0.8832 & -0.0257 & 0.1836 & 0.0333 & 0.8587 & 0.6305 & 0.7238 & \underline{21.4834} & \textbf{14.3622} & 3.83 \\
        \midrule
        SF & 0.8856 & -0.0241 & 0.1813 & 0.0336 & 0.8947 & \underline{0.6277} & 0.7279 & 21.2349 & 14.6864 & 3.56 \\
        CSF & \textbf{0.8873} & -0.0234 & \underline{0.1686} & \underline{0.0339} & \underline{0.9183} & 0.6305 & 0.7272 & 21.2381 & 14.7831 & 2.94 \\
        SF+LongTuning & 0.8857 & \underline{-0.0230} & \textbf{0.1680} & 0.0322 & 0.8160 & 0.6445 & \textbf{0.7300} & \textbf{21.5293} & \underline{14.4123} & \underline{2.78} \\
        CSF+LongTuning & \underline{0.8868} & \textbf{-0.0228} & 0.1691 & \textbf{0.0353} & \textbf{1.0039} & \textbf{0.6244} & \underline{0.7286} & 21.3137 & 14.6838 & \textbf{1.89} \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Consistency comparison with X-World~1.0 and training variants.} SF denotes Self Forcing, CSF denotes Connected Self Forcing, and LongTuning denotes long-horizon tuning. Best and second-best results in each column are shown in bold and underlined, respectively; missing values are excluded. App. denotes Mean Appearance Consistency, Decay denotes Mean Appearance Decay Rate, Ray denotes Mean Ray Residual (m), and Bits denotes the inter/intra encoded-size ratio. A less negative decay slope indicates slower loss of appearance similarity with temporal separation. Both PSNR quantities are measured in dB, and reconstruction MAE uses pixel intensity units (0--255). Avg. Rank is the mean rank across the nine metrics among the five models, with average ranks assigned to ties; lower is better.}
    \label{tab:consistency_stages}
\end{table}

==> backup/sections/introduction.tex <==

\section{Introduction}
\label{sec:introduction}

Since its release, X-World~1.0~\cite{xworld2026} has demonstrated
the practical value of controllable, multi-camera generative world
models for end-to-end autonomous driving.
By combining action-conditioned video generation, editable scene
controls, and streaming autoregressive rollouts, it provided a
concrete foundation for interactive driving simulation.
Its integration into XPENG's VLA~2.0 development pipeline has
supported closed-loop evaluation, online reinforcement learning,
and synthetic data generation, bringing learned simulation into
practical policy development and validation~\cite{xworld2026}.
Its approach to controllable multi-camera rollouts has also been
discussed in subsequent research~\cite{m4world2026}, contributing
an industrial example of the broader transition from open-loop
video synthesis to interactive driving simulation.

Building on this foundation, we introduce \textbf{X-World~1.6},
which advances the platform through three progressive developments.
We first strengthen the base model's understanding of driving
conditions and spatial relationships across cameras.
We then build on these capabilities to support \textbf{Virtual City}
through diverse forms of reference conditioning, broadening how
simulated scenes can be specified and initialized.
Finally, we develop a progressive post-training pipeline that
transforms the bidirectional, multi-step generator into a causal,
few-step model with improved temporal consistency, longer rollout
capability, and stronger alignment with human preferences.
A newly developed suite of evaluation metrics supports systematic
assessment and model iteration across these developments.

\textbf{Stronger foundational capabilities.}
Controllable driving video generation requires both structured
scene conditioning and coherent cross-view
modeling~\cite{gaia22025,magicdrivev22024}.
X-World~1.6 expands the base model's conditioning interface with
explicit controls for road markers and traffic lights (TFL),
enabling more precise specification of driving-relevant scene
semantics.
These additions complement the existing controls for ego motion,
traffic participants, and road structure, increasing the range
of scenarios that can be constructed and manipulated.
To strengthen cross-camera reasoning, we introduce
GeoPE, our multi-camera positional encoding module
inspired by the Plücker ray encoding~\cite{zhang2024cameras}.
%the geometry-aware attention of GTA~\cite{gta2023} and the relative camera encoding of PRoPE~\cite{prope2025,zhang2024cameras}.
GeoPE helps the model better capture spatial relationships
and visual correspondences across camera views.
Together, these advances provide a stronger foundation for
controllable and geometrically coherent multi-camera generation.

\textbf{Reference-conditioned generation for Virtual City.}
Geometric and visual references offer a practical interface
between scene assets and generative video
models~\cite{agarwal2026cosmos,cosmostransfer12025,gen3c2025,chen2026vggt}.
Building on the enhanced base model, we develop a family of
reference-conditioned models for Virtual City.
These models accommodate heterogeneous 2D and 3D reference inputs,
including point-cloud-based references, images rendered from
3D Gaussian scene representations~\cite{gaussiansplatting2023,chen2026quantifying,zhang2024gaussian},
and reference images, enabling different forms of scene control.
The model family also supports generating multi-camera future
videos from a \emph{single initial image}, expanding the ways
in which a driving simulation can be initialized.
Each reference-conditioning mode is currently implemented as a
separate model, tailored to its input format and control
requirements; integrating these capabilities into a unified
model remains a direction for future development.
This model family broadens scenario construction beyond complete
multi-camera recordings by allowing different sources of visual
and geometric information to guide generation.

\textbf{Progressive post-training for causal, few-step generation.}
Adapting bidirectional video generators to efficient causal
rollout is a key step toward interactive
simulation~\cite{causvid2024,causalforcingpp2026}.
Our post-training pipeline proceeds through
teacher forcing,
consistency distillation~\cite{consistencymodels2023},
and our \textbf{Connected Self Forcing (CSF)}~\cite{csf2026}.
Teacher forcing establishes causal prediction from historical
observations, consistency distillation reduces the denoising
budget, and CSF improves autoregressive generation under
self-generated histories.
Self Forcing~\cite{selfforcing2025} addresses the
training--inference mismatch by exposing the model to its own
rollouts, but detaching historical key--value caches interrupts
the backward connections between chunks.
Our CSF framework restores these connections, so that losses
on subsequent predictions can influence the computations that
generated earlier context.
This complements direct supervision of historical outputs with
feedback through their role in future generation, enabling
context to be optimized for both its own quality and its
usefulness to later predictions.

Prior studies highlight the importance of long-rollout training
and long-context supervision for sustained autoregressive
generation~\cite{longlive2025,contextforcing2026}.
Following the initial CSF stage, we introduce a teacher with a
longer temporal horizon to supervise \textbf{long CSF tuning},
further improving the model's ability to maintain quality over
extended rollouts.
% Within this framework, we combine the
% \textbf{distribution matching distillation (DMD)}
% objective~\cite{dmd2023} with an auxiliary \textbf{GAN branch},
% complementing distribution matching with adversarial supervision
% for visual quality~\cite{dmd22024}.
Feedback-driven refinement provides an additional route to
improving interactive world models beyond teacher-based
distillation~\cite{worldcompass2026}.
We therefore apply one-packed DiffusionNFT~\cite{zheng2026diffusionnft}
to further improve the causal model's generation quality and
align its outputs with human preferences.
Together, these stages strengthen the quality and temporal
reliability of the resulting few-step simulator.

Reliable evaluation is essential to assessing these advances
and guiding further development.
Existing benchmarks provide complementary perspectives on
video quality and intrinsic
faithfulness~\cite{vbench2023,vbench22025}, as well as world-model
capabilities such as controllability and physical
consistency~\cite{worldmodelbench2025,worldscore2025}.
To complement these perspectives, we develop a
\textbf{new suite of evaluation metrics tailored to multi-camera driving
world models}.
This suite provides a systematic basis for assessing model
capabilities, comparing modeling and training choices, and
guiding subsequent improvements.
Coupling this evaluation framework with advances in foundational
modeling, reference-conditioned scene generation, and causal
post-training further develops X-World as a platform for
interactive driving simulation.
\newpage


==> backup/sections/model_inference.tex <==
\section{Inference}
\label{sec:model_inference}

We deploy the four-step causal generator as a stateful inference service on
T-Head PPU M810E accelerators for closed-loop simulation. At each simulation
step, the simulator supplies the driving policy's updated ego motion and scene
controls, and the world model returns synchronized seven-camera observations
conditioned on the autoregressive history and clean KV-writing procedure of
Connected Self Forcing (Sec.~\ref{sec:connected_self_forcing}). Because a
single node serves multiple rollouts in parallel, we optimize aggregate
steady-state throughput, measured in synchronized seven-camera observations per
second per PPU across all active sessions.

\subsection{Stateful Autoregressive Execution}
\label{sec:inference_state}

Each simulation session maintains its own self-attention KV cache,
sampling-noise state, and causal VAE boundary state across requests. Initial
observations seed the history once at session creation; subsequent requests
update the control inputs and denoise the active two-latent (eight-frame)
causal block against this retained context. The service provides both a chunk
interface, which returns a full latent block per call, and a per-frame
interface for step-by-step closed-loop control. Under the per-frame interface,
the active causal block is re-denoised as new controls arrive within its
temporal span, and intermediate predictions overwrite the active block's KV
slots in place. Once all frames in the block have been emitted, the
clean-context pass $G_\theta^{\mathrm{KV}}$ (Sec.~\ref{sec:connected_self_forcing})
commits the finalized keys and values before advancing the window; intermediate
noisy predictions do not enter the history attended by later blocks.

The self-attention KV cache holds 13 latent frames per camera group: the first
three latent frames remain pinned as attention
sinks~\cite{xiao2024streamingllm}, while a 10-latent history window shifts in
place as generation advances. Device memory usage therefore stays constant
regardless of rollout length.

\subsection{Computation Reuse}
\label{sec:inference_residual_reuse}

\noindent\textbf{Session- and request-level conditioning.}
Static text embeddings and their per-layer cross-attention keys and values are
computed once at session initialization and reused throughout the rollout.
Request-level conditions that depend only on the target poses and controls
(GeoPE camera ray encodings, ego-motion modulation, structured-condition
tokens, traffic-light projections and spatial masks, and VAE-encoded 3DGS or
point-cloud renders in the 3D-conditioned variants) are encoded once per
request and reused across all four denoising steps and the
$G_\theta^{\mathrm{KV}}$ pass. For structured-condition cross-attention, the
cached keys and values are stored directly in the contiguous head-major layout
consumed by the attention matrix multiplications; camera groups without a
visible traffic light skip the traffic-light branch. In the reference-to-video
variant (Sec.~\ref{sec:r2v}), by contrast, the shared reference state exchanges
features with the video tokens at every layer and is recomputed at each
denoising step.

\noindent\textbf{Cross-request residual reuse.}
Consecutive requests of a session denoise closely related inputs, so the
runtime reuses DiT block residuals across successive generation chunks with
X-Cache~\cite{zeng2026xcache}. Each cache entry is indexed by denoising step
$s$, Transformer layer $\ell$, and prediction position within the causal block.
Let $h_{\ell,s}^{(n)}$ denote the input to layer $\ell$ at step $s$ of
generation $n$, and let $F_{\ell,s}$ denote the full block update. If
generation $m$ last recomputed this entry under conditions $c^{(m)}$, the
stored residual is
\begin{equation}
    r_{\ell,s}^{(m)}
    = F_{\ell,s}\!\left(h_{\ell,s}^{(m)};c^{(m)}\right)
      -h_{\ell,s}^{(m)},
    \label{eq:inference_cached_residual}
\end{equation}
and a subsequent generation $n$ that satisfies the reuse criterion bypasses the
block evaluation via
\begin{equation}
    \widetilde h_{\ell+1,s}^{(n)}
    = h_{\ell,s}^{(n)}+r_{\ell,s}^{(m)}.
    \label{eq:inference_residual_reuse}
\end{equation}
The reuse gate compares device-side fingerprints built from subsampled
spatiotemporal tokens, feature means, and action/camera conditions. A cached
residual is reused when the minimum cosine similarity exceeds an adaptive
per-layer EMA threshold and the maximum normalized spatial deviation stays
within bound. The cache warms on the initial pass; the first denoising step,
the first Transformer layer, and the $G_\theta^{\mathrm{KV}}$ clean-history
pass always run in full.

In our four-step, 30-layer DiT, $87$ of $120$ block evaluations per pass
($72.50\%$) fall outside the first denoising step and first layer; in open-loop
chunk generation, X-Cache reuses $53.5\%$ of blocks~\cite{zeng2026xcache}.
Under the per-frame closed-loop interface, each eight-frame causal block spans
eight requests across two latent positions: the eighth request runs a full pass
to commit clean KV via $G_\theta^{\mathrm{KV}}$, and the first request at each
latent position is rejected by the gate because its cached residual comes from
the preceding block. The remaining five of eight requests reuse nearly all 87
eligible blocks: the analytical ceiling is $(5/8)\times(87/120)=45.31\%$, and
the measured reuse rate across 12 concurrent sessions is
$45.22\%$.

\subsection{DiT Kernels on PPU}
\label{sec:inference_dit}

The 30-layer DiT (hidden dimension $3072$, 24 heads of dimension 128) executes
in BF16 and uses the SAIL implementation of
FlashAttention-3~\cite{shah2024flashattention3} for video self-attention. Around
the attention and feed-forward projections, we fuse the scale-and-shift
modulation after normalization and the gated residual update into single-launch
vectorized kernels (16-byte loads, 8 BF16 elements per thread). On the Q/K
path, a single kernel combines RMS normalization~\cite{zhang2019rmsnorm},
spatiotemporal rotary position embedding~\cite{su2021roformer}, and conversion
to BF16; the high-precision rotation arithmetic stays in registers rather than
materializing FP64 and complex Q/K tensors in device memory. In the
structured-condition cross-attention branch, query normalization writes directly in head-major order and masked
softmax runs as a single kernel.

\subsection{Causal VAE Execution}
\label{sec:inference_vae}

\noindent\textbf{Boundary snapshot and prefix decoding.}
For each camera, decoding conditions on the encoded last frame of the preceding
four-frame latent interval. After processing this boundary prefix, the decoder
snapshots its causal convolution states. Subsequent per-frame requests within
the same four-frame latent interval resume from this snapshot rather than
re-evaluating the boundary prefix, and the causal upsampling stages evaluate
only the temporal prefix required for the requested frame. Once the fourth
frame of the interval is emitted, it is re-encoded to establish the boundary
for the next interval.

\noindent\textbf{Channels-last layout and AIU 3D convolutions.}
Across the convolutional stages of the encoder and decoder, activations remain
in 3D channels-last (\texttt{NDHWC}) layout between layers, while the middle
attention block retains its reference layout. A fused input kernel constructs
causal padding, inserts cached history frames, extracts the next convolution
cache, and folds in preceding channel-wise RMS normalization and SiLU
activation in a single launch; companion kernels fuse per-channel bias addition
with residual shortcuts and execute $2\times$ nearest-neighbor upsampling
directly in \texttt{NDHWC}. For the dominant unpadded unit-stride
$3\times3\times3$ convolutions ($C\in\{256, 512, 1024\}$), we implement BF16
implicit-GEMM kernels using T-Head's \texttt{actlize} template library
($128\times256\times32$ threadblock tiles and $64\times64\times32$ warp tiles
across 8 warps), while remaining shapes run on acDNN. Hardware AIU load
instructions fetch convolution patches directly into on-chip tiles across a
4-stage pipeline without an explicit \texttt{im2col} buffer. Because matrix
instructions execute on 20 of the 64 compute units on the M810E, the kernel
launches a persistent grid across those 20 units.

\subsection{Concurrent Simulation Sessions}
\label{sec:inference_serving}

The serving runtime runs initialization, denoising, and VAE decoding in
separate worker processes. Admitted sessions use preallocated cache slots,
dedicated execution streams, and reusable pinned buffers for host-device
transfers. Each session stays bound to one denoiser for its entire rollout so
interleaved requests do not perturb its KV cache or random-number generator,
and binds to the least-loaded VAE decoder on its first decode request to
balance causal boundary snapshots across devices. On the return path, the
decoder converts output frames to 8-bit pixels on the PPU before
device-to-host transfer.

On a four-PPU M810E node, each device hosts one
denoiser and one VAE decoder, two devices additionally host initialization
workers, and each denoiser admits three sessions (12 concurrent sessions per
node). Co-locating a decoder on each PPU overlaps VAE kernel execution with
denoiser host dispatch. To keep three sessions within device memory, each
session's two X-Cache stores (one per latent position in the two-latent causal
block, where holding all $3\times29=87$ reusable BF16 residuals on device would
require 4.5~GiB per session or 13.4~GiB per denoiser) are kept in pinned host
memory and copied back asynchronously on reuse, limiting X-Cache device
overhead to 1.0~GiB per denoiser. Likewise, streaming the text encoder weights
from host memory on demand during session creation caps each initialization
worker at 4.1~GiB of HBM. In steady state, each denoiser occupies
$54.6\text{--}54.7$~GiB of HBM and each decoder occupies
$18.6\text{--}19.5$~GiB.

\subsection{Numerical Fidelity}
\label{sec:inference_exact}

In autoregressive generation, small floating-point discrepancies at individual
layers compound across denoising steps and closed-loop feedback: altering the
reduction order of the $3072$-channel normalization alone degrades a
closed-loop rollout to a worst-frame PSNR of 23.8~dB. The fused DiT and VAE
kernels therefore follow the reference reduction trees and intermediate BF16
rounding boundaries; they disable FMA contraction and match the reference
single-precision reciprocal semantics. Similarly, the AIU $3\times3\times3$
convolutions accumulate over channel groups and the 27 filter taps in FP32 in
the same order as acDNN before round-to-nearest-even conversion to BF16. Under
deterministic multi-stream BLAS workspaces and dedicated hardware queues per
session stream, all kernel and layout optimizations match the unfused reference
bit-for-bit across multi-session closed-loop rollouts. Cross-chunk residual
reuse is the only step that alters numerical values; across $1344$ generated
frames on closed-loop rollouts, the full runtime maintains a mean frame PSNR of
53.20~dB against the reference output (global PSNR 52.27~dB, minimum frame
PSNR 49.12~dB, and per-camera mean PSNR of $52.07\text{--}54.20$~dB across the
seven views).

\subsection{Inference Performance}
\label{sec:inference_performance}

Table~\ref{tab:ppu_inference} reports steady-state closed-loop serving
performance on a four-PPU M810E node running 12 concurrent sessions in BF16
with four denoising steps (two views at $512\times1024$, four at
$416\times512$, and one at $448\times896$; $2.30$~MPix per seven-camera
observation and $2248$ latent tokens per four-observation latent frame). Each
per-frame step covers condition preprocessing, DiT denoising, causal VAE
execution, and frame delivery.

\begin{table}[ht]
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\raggedright\arraybackslash}p{5.4cm}cccccccc@{}}
        \toprule
        & \multicolumn{2}{c}{Obs/s $\uparrow$} & \multicolumn{2}{c}{Denoiser (s) $\downarrow$} & \multicolumn{3}{c}{Step latency (s) $\downarrow$} & \\
        \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-8}
        Configuration & PPU & Node & P50 & Mean & P50 & Mean & P99 & Speedup $\uparrow$ \\
        \midrule
        Reference kernels & 0.156 & 0.625 & 5.96 & 5.92 & 19.04 & 18.68 & 23.80 & 1.00$\times$ \\
        + Channels-last VAE with fused causal input & 0.201 & 0.803 & 4.48 & 4.55 & 14.70 & 14.46 & 18.94 & 1.29$\times$ \\
        + Fused DiT kernels & 0.218 & 0.873 & 3.95 & 4.16 & 13.42 & 13.25 & 18.36 & 1.40$\times$ \\
        + AIU convolutions & \underline{0.237} & \underline{0.949} & \underline{3.69} & \underline{3.80} & \underline{12.49} & \underline{12.22} & \textbf{15.23} & \underline{1.52$\times$} \\
        + X-Cache & \textbf{0.320} & \textbf{1.281} & \textbf{2.10} & \textbf{2.62} & \textbf{8.69} & \textbf{8.94} & \underline{17.82} & \textbf{2.05}$\times$ \\
        \bottomrule
    \end{tabular*}
    \caption{Steady-state closed-loop serving throughput, server denoiser
    forward time, and per-session end-to-end step latency on a 4$\times$ PPU
    M810E node (12 concurrent sessions) with optimizations enabled
    cumulatively. Best and second-best values in each column are bold and
    underlined, respectively.}
    \label{tab:ppu_inference}
\end{table}

Kernel and layout optimizations alone raise throughput from 0.156 to
0.237~obs/s/PPU ($1.52\times$; $0.55$~MPix/s/PPU) and cut P99 step latency from
23.80~s to 15.23~s; eliminating 3D layout conversions and causal-padding copies
in the co-located VAE accounts for most of this gain. Adding X-Cache brings
steady-state throughput to 0.320~obs/s/PPU ($2.05\times$; $0.74$~MPix/s/PPU)
and reduces median denoiser time from 3.69~s to 2.10~s, while P99 step latency
(17.82~s) reflects the full passes executed on clean-KV commit steps and
latent-position transitions.


==> backup/sections/modeldesign.tex <==
\section{Method}

This section should present the proposed method at a level that allows readers to understand and reproduce the core idea.
Start with a short overview of the full pipeline, then introduce each component in the order it is used.

\subsection{Problem Formulation}

Define the inputs, outputs, assumptions, and notation.
For example, let $x$ denote the input, $y$ denote the target output, and $f_\theta$ denote the model or algorithm being optimized.
Clarify whether the setting is supervised, self-supervised, generative, interactive, or analytical.

\subsection{System Overview}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{pngs/image1.png}
    \caption{\textbf{Method overview.} Replace this placeholder with a diagram of the proposed pipeline, including inputs, major modules, and outputs.}
    \label{fig:method_overview}
\end{figure}

Describe the major components shown in Figure~\ref{fig:method_overview}.
Keep this subsection conceptual; details such as architecture, losses, and implementation choices can be moved to later subsections.

\subsection{Core Module}

Explain the main technical component.
State what problem it solves, what information it consumes, and what representation or prediction it produces.
If the method uses a neural architecture, describe the backbone, conditioning signals, and output heads.
If the method is not neural, describe the algorithmic stages and decision rules.

\subsection{Objective}

Provide the training or optimization objective.
Use equations for important losses and define each term immediately after it appears:
\begin{equation}
    \mathcal{L} = \lambda_1 \mathcal{L}_{\mathrm{main}} + \lambda_2 \mathcal{L}_{\mathrm{reg}}.
\end{equation}
Here, $\mathcal{L}_{\mathrm{main}}$ is the primary task loss and $\mathcal{L}_{\mathrm{reg}}$ is an optional regularization term.

\subsection{Implementation Details}

Summarize implementation choices that are needed for reproducibility, including model size, optimizer, learning rate schedule, batch size, hardware, and relevant preprocessing.
Move lengthy details to the appendix when they interrupt the main narrative.


==> backup/sections/modeltraining.tex <==
\section{Training}

Our training pipeline consists of bidirectional pretraining followed by autoregressive post-training, as illustrated in Fig.~\ref{fig:training_pipeline}. After adapting the video generation backbone to the egocentric multi-view driving setting (Sec.~\ref{sec:training_setup}), we use teacher forcing (Sec.~\ref{sec:teacher_forcing}) to obtain a causal model and consistency distillation (Sec.~\ref{sec:causal_consistency_distillation}) to adapt it for few-step denoising. We further distill the model through Connected Self Forcing (Sec.~\ref{sec:connected_self_forcing}), using self-generated histories as context. We then extend the training horizon by continuing CSF training with a bidirectional teacher fine-tuned on longer sequences (Sec.~\ref{sec:long_horizon_tuning}). Finally, we apply reward-guided reinforcement learning through One Packed NFT to improve visual quality and trajectory accuracy in generated videos (Sec.~\ref{sec:diffusion_rl}).

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/Training_Pipeline.pdf}
    \caption{\textbf{Training pipeline.} (01) Bidirectional pretraining uses full attention in two stages, with high and then low condition dropout. (02) Teacher forcing (TF) uses concatenated ground-truth and noisy sequences with causal attention. (03) Causal consistency distillation retains this input structure and uses a frozen TF teacher to adapt the model for few-step generation. (04) Connected Self Forcing (CSF) trains with self-generated histories under distribution matching distillation (DMD) supervision and reconnects cross-chunk gradients through shortcut replay to support few-step streaming inference over long horizons. (05) Long-horizon tuning continues CSF training using a bidirectional teacher fine-tuned on longer sequences. (06) Reinforcement learning further optimizes the causal generator using Causal One Packed NFT with visual and trajectory rewards.}
    \label{fig:training_pipeline}
\end{figure}

\subsection{Bidirectional Pretraining}
\label{sec:training_setup}

We pretrain bidirectional video models on synchronized seven-view driving videos in two stages. Starting from the pretrained Wan2.2-TI2V-5B backbone~\cite{wan2025}, we train the model to accommodate diverse conditioning inputs, following the architectural designs described in Sec.~\ref{sec:method}. The model supports different forms of scene conditioning, including initial images for image-to-video (I2V) generation, reference images for reference-to-video (R2V) generation, reference videos for reference-video-to-video (RV2V) generation, and 3D scene representations such as 3DGS renderings and point clouds. Depending on the model configuration, additional conditions include text descriptions, ego actions, structured scene controls (e.g., dynamic agents, lanes, road markers, and traffic-light states), and target camera configurations. All models follow the same training formulation, with $c$ denoting the conditioning inputs and $\theta$ the parameters of each independently trained model.

Let $x_0=\{x_0^v\}_{v=1}^{7}$ denote the clean VAE latents of a synchronized seven-view video, where $v$ indexes the camera view. Following Rectified Flow~\cite{liu2022flow}, we sample a noise timestep $\tau$ and construct
\begin{equation}
x_\tau=(1-\sigma_\tau)x_0+\sigma_\tau\epsilon,
\qquad
\epsilon\sim\mathcal N(0,I),
\end{equation}
where $\sigma_\tau$ is the noise level shared across all seven views, with Gaussian noise sampled independently for each view. The bidirectional DiT processes the noisy video latents with full temporal attention and predicts the corresponding flow velocity. Denoting the conditions after random dropout by $\tilde c$, we optimize the timestep-weighted flow-matching objective:
\begin{equation}
\mathbb E\left[
    w(\tau)\,
    \operatorname{MSE}\left(
        v_\theta(x_\tau,\tau;\tilde c),\,
        \epsilon-x_0
    \right)
\right],
\end{equation}
where $v_\theta$ denotes the predicted flow velocity and $w(\tau)$ is the timestep-dependent loss weight. The MSE is averaged over all latent elements across the seven views. During pretraining, we optimize the DiT while keeping the VAE and text encoder frozen.

We adopt a two-stage condition-dropout schedule to progressively adjust the emphasis on conditional generation. In the first stage, we apply high dropout probabilities to individual conditioning branches, encouraging the model to learn from incomplete combinations of conditions and reducing over-reliance on any fixed set of inputs. When all droppable conditions are absent or dropped, we additionally apply temporal latent inpainting. Specifically, randomly selected latent time positions are kept clean with zero timesteps and velocity targets, allowing the model to learn from sparse temporal observations. In the second stage, we continue training from the first-stage checkpoint with reduced condition-dropout probabilities, exposing the model more frequently to the provided controls to strengthen conditional adherence. Temporal inpainting is disabled, while the bidirectional architecture and flow-matching objective remain unchanged. The resulting bidirectional checkpoints provide initialization for subsequent causal training and serve as real-score teachers for distribution matching distillation.

\subsection{Autoregressive Post Training}
\textbf{Teacher-Forcing Adaptation}.
\label{sec:teacher_forcing}
To adapt the bidirectional model for causal video generation, we initialize it from the second-stage pretraining checkpoint and apply teacher forcing. Full temporal attention is replaced with a block-causal attention mask, while bidirectional attention is preserved within each chunk. Specifically, clean ground-truth (GT) video latents and their noisy counterparts at corresponding temporal positions are concatenated and processed in a single forward pass, enabling parallel training across chunks.

Let $x_0^{(i)}$ and $x_{\tau_i}^{(i)}$ denote the clean and noisy latents of chunk $i$, respectively. The visible context for each noisy chunk is defined as
\begin{equation}
\operatorname{Context}_{\mathrm{TF}}\left(x_{\tau_i}^{(i)}\right)
= \left\{x_0^{(j)}\mid j<i\right\}
\cup \left\{x_{\tau_i}^{(i)}\right\},
\end{equation}
where $\tau_i$ is independently sampled for each chunk and shared across its seven synchronized views. Accordingly, each noisy chunk attends to preceding GT chunks and its own noisy tokens, without accessing the current GT chunk or future chunks. The clean GT branch is also causally masked to prevent future information leakage.

Training retains the timestep-weighted flow-matching objective from Sec.~\ref{sec:training_setup}, with supervision applied only to the noisy branch and clean GT latents serving as historical context. The resulting causal model provides the initialization for subsequent consistency distillation.

\textbf{Causal Consistency Distillation}.
\label{sec:causal_consistency_distillation}
Following Causal Forcing++~\cite{causalforcingpp2026}, we apply Causal Consistency Distillation (CD)~\cite{consistencymodels2023} to enable few-step generation. Both the trainable student and a frozen causal teacher are initialized from the TF checkpoint, retaining the teacher-forcing input structure and attention mask.

For a sampled noise timestep $\tau$, the frozen TF teacher performs one Euler denoising step with classifier-free guidance (CFG) to construct an adjacent state at a lower noise level:
\begin{equation}
x_{\tau'}^{(i)} = x_\tau^{(i)}
+ (\sigma_{\tau'}-\sigma_\tau)\,
  v_{\mathrm{TF}}^{\mathrm{CFG}}\left(
    x_\tau^{(i)},\tau; h_{\mathrm{GT}}^{(i)},c
  \right),
\qquad \sigma_{\tau'}<\sigma_\tau,
\end{equation}
where $h_{\mathrm{GT}}^{(i)}$ denotes the preceding GT chunks. The same pair of adjacent noise timesteps is shared across all chunks and synchronized camera views.

The student and its exponential moving average (EMA) counterpart predict the clean endpoint from $x_\tau^{(i)}$ and $x_{\tau'}^{(i)}$, respectively, under the same GT history and conditioning inputs. The consistency loss is defined as
\begin{equation}
\mathcal L_{\mathrm{CD}} = \mathbb E\left[
  \operatorname{MSE}\left(
    \hat x_{0,\theta}^{(i)}(\tau),
    \operatorname{sg}\left[
      \hat x_{0,\bar\theta}^{(i)}(\tau')
    \right]
  \right)
\right],
\end{equation}
where $\bar\theta$ denotes the EMA parameters and $\operatorname{sg}$ indicates stop-gradient. The EMA weights of the distilled student are used to initialize the generator for subsequent Connected Self Forcing.

\textbf{Connected Self Forcing.}
\label{sec:connected_self_forcing}
Following consistency distillation, the causal generator is further optimized using our Connected Self Forcing (CSF)~\cite{csf2026}, building on Self Forcing~\cite{selfforcing2025}. Unlike the preceding stages that rely on ground-truth (GT) histories, CSF trains on self-generated autoregressive rollouts. Conditioned on the model-specific scene inputs and controls, the generator produces synchronized seven-view video chunks through few-step denoising, using previously generated chunks as visual context. Each generated chunk is subsequently processed by a KV-writing pass ($G_\theta^{\mathrm{KV}}$), which shares parameters with the generator ($G_\theta$), to update the historical KV cache for subsequent generation.

The generated rollouts are optimized using Distribution Matching Distillation (DMD)~\cite{dmd2023,dmd22024}. A frozen bidirectional real-score teacher from pretraining provides distributional supervision, while a trainable fake-score model tracks the generator distribution. DMD evaluates re-noised generated latents using both score models, providing direct gradients to the generated chunks.

In standard Self Forcing, historical KV caches are detached to reduce memory consumption, preventing gradients from later chunks from reaching earlier generation computations. CSF addresses this limitation through \textbf{Shortcut Gradient Replay}. During training, the autoregressive rollout is detached while retaining the states required for replay. Given the DMD gradient from a later chunk, its denoising computation is replayed with selected historical KV states made differentiable, recovering gradients on these caches. The gradients are then propagated through the corresponding KV-writing computations to the historical generated chunks, and further through their replayed denoising computations to update the shared generator parameters. The resulting training signal for a historical chunk $j$ combines direct DMD supervision with cross-chunk feedback:
\begin{equation}
\mathbf g_{\mathrm{DMD}}^{(j)}
+ \mathbf g_{\mathrm{cross}}^{(j)},
\end{equation}
where $\mathbf g_{\mathrm{cross}}^{(j)}$ aggregates feedback from subsequent chunks through the replayed historical context. This avoids retaining the full autoregressive computation graph, while allowing historical chunks to be optimized for both their own generation quality and their contribution to future predictions. Shortcut replay is used only during training, leaving the causal inference procedure unchanged.

\textbf{Long-Horizon Tuning.}
\label{sec:long_horizon_tuning}
To improve the plausibility of long-horizon scene evolution and mitigate visual hallucinations, we further extend the training horizon. We first fine-tune the bidirectional teacher on longer synchronized seven-view video sequences, retaining the bidirectional attention and flow-matching objective described in Sec.~\ref{sec:training_setup}. This extends the temporal range of the teacher's distributional supervision.

We then continue Connected Self Forcing from the previously trained generator checkpoint, replacing the original real-score teacher with the extended bidirectional model. Both the student rollout length and teacher supervision window are increased, while retaining few-step denoising, self-generated histories, DMD supervision, and Shortcut Gradient Replay. This exposes the generator to longer autoregressive trajectories and provides training signals over extended temporal contexts, without modifying its causal architecture or inference procedure.

\subsection{Efficient RL for Autoregressive Models}
\label{sec:diffusion_rl}

\textbf{One Packed NFT}.
\label{sec:one_packed_nft}
We adopt DiffusionNFT~\cite{zheng2026diffusionnft}, which trains on forward-noised versions of generated samples without backpropagating through the sampling process. Our autoregressive model conditions each video block on previously denoised blocks. If all blocks are jointly noised for parallel training, a standard causal mask still exposes each target block to noisy history, creating a mismatch with the conditioning used during generation. To address this, One Packed NFT separates the encoding of clean history into attention keys and values (KV) from the prediction of noisy target blocks. This allows multiple target blocks to be evaluated together while each remains conditioned on its corresponding clean history.

The frozen old policy generates a shared clean prefix $P$ and $K$ candidate suffixes. For a single candidate, we write $Z=(z_b,\ldots,z_E)$, omitting the candidate index throughout. Samples and rewards remain fixed during inner updates. Each suffix block is independently noised as $x_j=(1-\sigma_t)z_j+\sigma_t\epsilon$, with its own timestep and noise; the prefix remains clean. Current, old, and reference encode these samples with their respective parameters into detached, per-layer KV banks. Each clean block attends only to itself and its permitted past at every layer.

Packed query block $j$ accesses
\begin{equation}
\mathcal S_j
=
\mathcal W_j\!\left(
\operatorname{Tok}(P\mathbin{\Vert}z_{b:j-1})
\cup
\operatorname{Tok}(x_j)
\right),
\label{eq:block_visibility}
\end{equation}
where $\Vert$ denotes concatenation, $\operatorname{Tok}$ denotes tokens, and $z_{b:j-1}$ is empty for $j=b$. The operator $\mathcal W_j$ enforces the original sink/window constraints. Historical K/V come from the clean bank, while each query supplies its own noisy K/V. Its clean target, future clean blocks, and other noisy blocks remain masked.

Sequential evaluation requires $H=E-b+1$ target calls per policy role and candidate batch, interleaved with clean-cache extension. We construct the clean bank first and evaluate all $H$ targets in one packed call, aggregating their losses into the NFT objective. Temporal positions, camera embeddings, and structured conditions are retained. Gradients flow only through the current query path.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/One_Packed_NFT.pdf}
    \caption{
    \textbf{One Packed NFT.}
    Both alternatives use the same frozen old trajectories.
    (a) Sequential evaluation interleaves target prediction with clean-cache extension.
    (b) A detached clean KV bank enables packed target prediction with preserved causal conditioning.
    Filled mask entries admit past clean keys and each target's own noisy keys, subject to the original sink/window constraints.
    Policy roles and candidate indices are omitted in the comparison panels.
    }
    \label{fig:one_packed_nft}
\end{figure*}

\textbf{Joint Visual-Motion NFT Objective}.
\label{sec:joint_reward_nft}
We evaluate frozen trajectories with HPSv3~\cite{ma2025hpsv3} for visual preference and a fixed inverse dynamics model (IDM) for ego-motion consistency. HPSv3 scores are averaged over frames associated with each temporal latent and camera; IDM rewards measure agreement between inferred and prescribed ego motion. Each reward is independently standardized across valid candidates at each latent and clipped to $[-C,C]$, yielding advantages $A_H$ and $A_I$. Visual normalization is camera-specific, while motion advantages are broadcast across views. We form $A_{\mathrm{mix}}=\alpha_H A_H+\alpha_I A_I$, with nonnegative weights summing to one and $C>0$.

Following DiffusionNFT, the implicit branches are $v^\pm=v_o\pm\beta(v_\theta-v_o)$, where $v_\theta,v_o$ are current and frozen old velocity predictions and $\beta>0$. With interpolation target velocity $v_{\mathrm{target}}=\epsilon-z$ and preference $\pi=(1+A_{\mathrm{mix}}/C)/2$, the policy loss is
\begin{equation}
\ell_{\mathrm{NFT}}
=
\sigma_t^2\left[
\pi\|v^+-v_{\mathrm{target}}\|_{\mathrm{mse}}^2
+
(1-\pi)\|v^--v_{\mathrm{target}}\|_{\mathrm{mse}}^2
\right].
\label{eq:mixed_nft_loss}
\end{equation}
The factor $\sigma_t^2$ preserves the clean-sample reconstruction objective. We aggregate target losses and add a frozen reference penalty,
\begin{equation}
\mathcal L_{\mathrm{joint}}
=
\mathcal R_{\mathrm{policy}}(\ell_{\mathrm{NFT}})
+
\lambda_{\mathrm{ref}}\mathcal R_{\mathrm{target}}\!\left(
\|v_\theta-\operatorname{sg}(v_{\mathrm{ref}})\|_{\mathrm{mse}}^2
\right),
\label{eq:joint_objective}
\end{equation}
where $\lambda_{\mathrm{ref}}\geq0$ and $\operatorname{sg}$ denotes stop-gradient. 
